Galois sections and $p$-adic period mappings

Let $K$ be a number field not containing a CM subfield. For any smooth projective curve $Y/K$ of genus $\geq2$, we prove that the image of the "Selmer" part of Grothendieck's section set inside the $K_v$-rational points $Y(K_v)$ is finite for every finite place $v$. This gives an unconditional verification of a prediction of Grothendieck's section conjecture. In the process of proving our main result, we also refine and extend the method of Lawrence and Venkatesh, with potential consequences for explicit computations.

==> prelims.tex <==
\section{Preliminaries: Galois representations and $(\varphi,N,G_v)$-modules}

We collect in this section several results on local and global Galois results which will be used in the sequel. This is essentially a rephrasing of the material in \cite[\S2]{LV}, except that we treat a few subjects -- $(\varphi,N,G_v)$-modules and self-conjugate places -- in greater generality. This is so that we can avoid good reduction hypotheses when we set up the machinery of Lawrence--Venkatesh, which will be important in our proof of the main theorem. The reader may wish to skip this section on a first reading, referring back to it as needed.

\subsection{Global Galois representations and purity}

We keep notation as in~\S\ref{ss:notation}, so~$K$ is a number field with absolute Galois group~$G_K$.

\begin{defi}[Purity]
Let~$u$ be a place of the number field~$K$ not dividing~$p\infty$. We say that an unramified representation~$V$ of~$G_u$ is \emph{pure of weight~$n\in\bZ$} just when the characteristic polynomial of the geometric Frobenius has coefficients in~$\bQ$, and all of its roots in~$\bC$ have absolute value~$q_u^{n/2}$ where~$q_u$ denotes the order of the residue field of~$K_u$. When $n\geq0$, we say moreover that~$V$ is \emph{integral} just when the monic characteristic polynomial of the geometric Frobenius has coefficients in~$\bZ$.

We say that a representation~$V$ of~$G_K$ is \emph{unramified and pure} (resp.\ \emph{unramified, pure and integral}) at~$u$ just when its restriction to the decomposition group~$G_u$ is.
\end{defi}

\begin{ex}\label{ex:cohomology_pure}
Let~$X/K$ be a smooth proper variety over the number field~$K$. Then there is a finite set~$T$ of places of~$K$ outside which~$X$ has good reduction, i.e.\ $X$ is the generic fibre of a smooth proper~$\cO_{K,T}$-scheme~$\fX$. Enlarging~$T$ if necessary, we may assume that it contains all places dividing~$p\infty$.

Then for all~$n\geq0$, the \'etale cohomology $\rH^n_\et(X_{\Kbar},\bQ_p)$ is unramified, pure and integral of weight~$n$ at all places outside~$T$. Unramifiedness follows from smooth proper base change for \'etale cohomology, and purity and integrality from Deligne's proof of the Weil Conjectures \cite[Th\'eor\`eme~1.6]{deligne:weil_i}.
\end{ex}

It turns out that purity imposes strong restrictions on a Galois representation~$V$. For example, it was proved by Faltings \cite[Satz~5]{faltings:endlichkeitssaetze}\cite[Lemma~2.3]{LV} that for a given dimension~$d$, weight~$n\geq0$ and finite set~$T$ of places of~$K$, there are only finitely many $d$-dimensional semisimple representations~$V$ of~$\Gal_K$ which are unramified, pure and integral of weight~$n$ outside~$T$. The tricky word here is ``semisimple'': it is in general quite easy to produce Galois representations which are unramified, pure and integral outside a finite set of primes (see Example~\ref{ex:cohomology_pure}), but it is very hard to show that these representations are semisimple. Even in the case of an abelian variety~$A/K$, semisimplicity of~$\rH^n_\et(A_{\Kbar},\bQ_p)$ is part of the Tate Conjecture, and is only known thanks to work of Faltings~\cite[Resultat~(a)]{faltings:endlichkeitssaetze}. 

\begin{ex}
Non-semisimple representations of $\Gal_\bQ$ that are pure of weight $0$ and integral outside $p$ can be obtained via the additive character $\psi\colon\pi_1(\Spec(\bZ[1/p])) \to \bZ_p$ obtained by the $p$-adic cyclotomic character composed with the $p$-adic logarithm, namely as
\[
\rho\colon\Gal_\bQ \to \GL_2(\bQ_p), \quad \rho(\sigma) =
\begin{pmatrix}
1 & \psi(\sigma) \\
& 1
\end{pmatrix}.
\]
%This unipotent representation is not a de Rham representation.
\end{ex}

Instead of using Faltings' Lemma~\cite[Lemma~2.3]{LV}, we will use a variant thereof for symplectic representations.

\begin{defi}[$\Sp$-irreducibility, {\cite[p10]{LV}}]\label{def:sp-irred}
A symplectic representation~$(V,\omega)$ of~$\Gal_K$ is called \emph{$\Sp$-irreducible} just when~$V$ has no non-zero $\Gal_K$-stable isotropic subspace (subspace on which~$\omega$ vanishes). This amounts to say that the representation does not factor over a nontrivial parabolic subgroup of the symplectic group~$\Sp$.
\end{defi}

\begin{lem}[{\cite[Lemma~2.6]{LV}}]\label{lem:faltings_symplectic}
Let~$T$ be a finite set of places of~$K$ containing all places dividing~$p\infty$, and $n,d$ non-negative integers. Then there are, up to isomorphism, only finitely many $\Sp$-irreducible symplectic representations $(V,\omega)$ of~$\Gal_K$ which have rank~$2d$ and are unramified, pure and integral of weight~$n$ outside~$T$.
\end{lem}

\begin{rmk}
Our using Lemma~\ref{lem:faltings_symplectic} differs slightly from the argument in~\cite{LV}, which instead uses Faltings' Lemma~\cite[Lemma~2.3]{LV} in the original form. This leads to slight improvements in certain estimates at one stage of the proof \todo{ref}.
\end{rmk}

\subsection{Local Galois representations and $(\varphi,N,G_v)$-modules}

While the theory of global Galois representations is very complicated, the theory of local Galois representations is much better understood, thanks to the work of Fontaine. Let us keep notation as in~\S\ref{ss:notation}, so that~$K_v$ is a finite extension of~$\bQ_p$ with algebraic closure~$\Kbar_v$, and~$\bQ_p^\nr$ is the maximal unramified extension of~$\bQ_p$ contained in~$\Kbar_v$. We will recall some of the basic theory of representations of the absolute Galois group~$G_v$ of~$K_v$.

\subsubsection{De Rham representations}

Fontaine's theory identifies a certain class of $G_v$-representations, called the \emph{de Rham representations}, which turns out to contain all representations coming from geometry. Fontaine defines a certain $\Kbar_v$-algebra~$\sB_\deR$, called the \emph{ring of de Rham periods}, which is endowed with an action of the Galois group~$G_v$ restricting to the tautological action on~$\Kbar_v$. For a representation~$V$ of~$G_v$, one has the $K_v$-vector space 
\[
\sD_\deR(V):=(\sB_\deR\otimes_{\bQ_p}V)^{G_v},
\]
whose $K_v$-dimension is at most $\dim_{\bQ_p}(V)$. One says that~$V$ is \emph{de Rham} just when equality holds: 
\[
\dim_{K_v}(\sD_\deR(V))=\dim_{\bQ_p}(V).
\]
The de Rham representations form a full $\otimes$-subcategory 
\[
\Rep_{\bQ_p}^\deR(G_v)\subseteq\Rep_{\bQ_p}(G_v)
\]
closed under subobjects \cite[Th\'eor\`eme~3.8(ii)]{fontaine:representations_semi-stables}, and the assignment $V\mapsto\sD_\deR(V)$ is $\otimes$-functorial in de Rham representations~$V$.

Moreover, the period ring $\sB_\deR$ is a complete discretely valued field and as such carries an exhaustive, separated $G_v$-stable filtration by fractional ideals of its valuation ring. %compatible with the algebra structure, 
This induces a $K_v$-linear filtration on $\sD_\deR(V)$ for every %de Rham 
representation~$V$. This is called the \emph{Hodge filtration} and denoted~$\rF^\bullet = \rF^\bullet V$. The Hodge filtration is $\otimes$-functorial in~$V$ for de Rham representations, see 
\cite[\S3.8]{fontaine:representations_semi-stables}.

It turns out that de Rham representations are ubiquitous in algebraic geometry over~$K_v$: any representation arising as the \'etale cohomology of a smooth proper variety is de Rham, and~$\sD_\deR$ of such a representation recovers the de Rham cohomology with its Hodge filtration. This is Fontaine's $C_\deR$ Conjecture, and a precise statement is as follows. 

\begin{thm}[$C_\deR$ Conjecture, {\cite[Theorem~8.1]{faltings:crystalline_cohomology}, \cite[Theorem~A1]{tsuji:c_st_survey}}]\label{thm:c_dr}
Let~$K_v$ be a finite extension of~$\bQ_p$ with algebraic closure $\Kbar_v$, and let~$X/K_v$ be a smooth proper variety. Then the following holds.
\begin{enumerate}[label={\emph{(\arabic*)}}]
\item
For all $n \geq0$, the $G_v$-representation $\rH^n_\et(X_{\Kbar_v},\bQ_p)$ is de Rham.
\item 
There is a natural $K_v$-linear comparison isomorphism
\[
c_\deR\colon \sD_{\deR,v}(\rH^n_\et(X_{\Kbar_v},\bQ_p))\xrightarrow\sim\rH^n_\deR(X/K_v)
\]
which is strictly compatible with the Hodge filtration on both sides. 
\item\label{thmpart:c_dr_compatibilities} 
The isomorphisms $c_\deR$ are compatible with all the natural constructions in cohomology: they are natural in~$X$ and~$K_v$, and are compatible with cup products, K\"unneth decompositions\footnote{Compatibility with K\"unneth decompositions is not stated in \cite{tsuji:c_st_survey}. However, it follows automatically from compatibility with cup products and functoriality, since the K\"unneth isomorphism $\rH^\bullet(X)\otimes\rH^\bullet(Y)\xrightarrow\sim\rH^\bullet(X\times Y)$ for a Weil cohomology theory $\rH^\bullet$ is the unique cga map which restricts to the maps $\rH^\bullet(X)\rightarrow\rH^\bullet(X\times Y)$, $\rH^\bullet(Y)\rightarrow\rH^\bullet(X\times Y)$ induced by the product projections.}, trace maps, Poincar\'e duality, pushforward, cycle class maps and Chern classes.
\end{enumerate}
\end{thm}

%%% Old versionn:
%\begin{thm}[$C_\deR$ Conjecture, {\cite[Theorem~8.1]{faltings:crystalline_cohomology}, \cite[Theorem~A1]{tsuji:c_st_survey}}]
%Let~$K_v$ be a finite extension of~$\bQ_p$ with algebraic closure $\Kbar_v$. Let~$L_w$ be a finite extension of~$K_v$ contained in~$\Kbar_v$ with absolute Galois group~$G_w \subseteq G_v$; let $X/L_w$ be a smooth proper variety and let~$X_{\Kbar_v}$ denote the base change of~$X$ from~$L_w$ to~$\Kbar_v$.
%
%Then for all $n\geq0$, the $G_w$-representation $\rH^n_\et(X_{\Kbar_v},\bQ_p)$ is de Rham, and there is a canonical $L_w$-linear comparison isomorphism
%\[
%c_\deR\colon\sD_{\deR,w}(\rH^n_\et(X_{\Kbar_v},\bQ_p))\xrightarrow\sim\rH^n_\deR(X/L_w)
%\]
%which is strictly compatible with the Hodge filtration, where $\sD_{\deR,w}(-)=(\sB_\deR\otimes_{\bQ_p}-)^{G_w}$. 
%
%Moreover, the isomorphisms $c_\deR$ are compatible with all the natural constructions in cohomology: they are natural in~$X$ and~$L_w$, and are compatible with cup products, K\"unneth decompositions\footnote{Compatibility with K\"unneth decompositions is not stated in \cite{tsuji:c_st_survey}. However, it follows automatically from compatibility with cup products and functoriality, since the K\"unneth isomorphism $\rH^\bullet(X)\otimes\rH^\bullet(Y)\xrightarrow\sim\rH^\bullet(X\times Y)$ for a Weil cohomology theory $\rH^\bullet$ is the unique cga map which restricts to the maps $\rH^\bullet(X)\rightarrow\rH^\bullet(X\times Y)$, $\rH^\bullet(Y)\rightarrow\rH^\bullet(X\times Y)$ induced by the product projections.}, trace maps, Poincar\'e duality, pushforward, cycle class maps and Chern classes.
%\end{thm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{$(\varphi,N,G_v)$-modules} 

One of the most fundamental results in $p$-adic representation theory is that the category of de Rham representations can be described equivalently in terms of explicit semilinear-algebraic objects known as \emph{filtered discrete $(\varphi,N,G_v)$-modules}. We recall the definition from \cite{fontaine:representations_semi-stables}.

The prime-to-$p$ cyclotomic character of $K_v$ yields a  homomorphism
\[
G_v \to \Gal(\bQ_p^\nr/\bQ_p) = p^{\hZ} \subseteq (\hZ/\bZ_p)^\times,
\]
which determines a continuous discrete action of $G_v$ on the field $\bQ_p^\nr$. 

\begin{defi}[{\cite[\S4.2.1]{fontaine:representations_semi-stables}}]
\label{def:discretephiNGvmodule}
A \emph{$(\varphi,N,G_v)$-module} is a $\bQ_p^\nr$-vector space $D$ endowed with:
\begin{enumerate}[label=(\roman*)]
	\item a bijective semilinear \emph{crystalline Frobenius} $\varphi$ (acting as absolute Frobenius on scalars),
	\item a $\bQ_p^\nr$-linear \emph{monodromy operator} $N$, and
	\item a semilinear action of the Galois group $G_v$ (with $G_v$ acting on scalars $\bQ_p^\nr$ as recalled above).
\end{enumerate}
These are required to satisfy:
\begin{enumerate}[label=(\roman*),resume]
	\item $N\circ\varphi=p\cdot\varphi\circ N$; and
	\item both $N$ and $\varphi$ commute with the action of $G_v$.
\end{enumerate}
The \emph{dimension} of $D$ is its dimension as $\bQ_p^\nr$-vector space.
\smallskip

A \emph{filtered discrete $(\varphi,N,G_v)$-module}\todo{can we ditch the word ``discrete'' now?}\todo{Also, do we like $(D,D_{K_v},c_\BO)$ or $(D_\pst,D_\deR,c_\BO)$?} is a tuple~$D=(D,D_{K_v},c_\BO)$ consisting of a $(\varphi,N,G_v)$-module~$D$, a $K_v$-vector space~$D_{K_v}$ endowed with an exhaustive, separated, decreasing $K_v$-linear filtration~$\rF^\bullet$, and a $\Kbar_v$-linear $G_v$-equivariant \emph{comparison isomorphism}
\[
c_\BO\colon \Kbar_v\otimes_{\bQ_p^\nr}D \xrightarrow\sim \Kbar_v\otimes_{K_v}D_{K_v} \,.
\]
The filtration~$\rF^\bullet$ is referred to as the \emph{Hodge filtration} on~$D$.

The collection of all filtered discrete~$(\varphi,N,G_v)$-modules forms a $\otimes$-category $\MF(\varphi,N,G_v)$ with respect to the obvious morphisms and tensor products.
\end{defi}

\begin{rmk}
	The above definition of filtered discrete~$(\varphi,N,G_v)$ is slightly non-standard, but equivalent to the standard definition \cite[\S4.3.2]{fontaine:representations_semi-stables}. Usually, a filtered discrete~$(\varphi,N,G_v)$-module is defined to be a $(\varphi,N,G_v)$-module~$D$ such that the point-stabilisers of the $G_v$-action on~$D$ are open in~$G_v$, endowed with an exhaustive, separated, decreasing filtration~$\rF^\bullet$ of~$\Kbar_v\otimes_{\bQ_p^\nr}D$ by $G_v$-invariant $K_v$-subspaces.
	
	This definition is equivalent to Definition~\ref{def:discretephiNGvmodule}, in the sense that they define canonically $\otimes$-equivalent $\otimes$-categories. Indeed, if~$(D,D_{K_v},c_\BO)$ is a filtered discrete $(\varphi,N,G_v)$-module in the sense of Definition~\ref{def:discretephiNGvmodule}, then the comparison isomorphism~$c_\BO$ ensures that the action of~$G_v$ on~$D$ has open point-stabilisers, and the filtration on~$\Kbar_v\otimes_{\bQ_p^\nr}D$ given by pulling back the Hodge filtration on~$D_{K_v}$ along~$c_\BO$ makes~$D$ into a filtered discrete $(\varphi,N,G_v)$-module in the sense of~\cite[\S4.2.2]{fontaine:representations_semi-stables}. Conversely, if~$D$ is a filtered discrete $(\varphi,N,G_v)$-module in the sense of~\cite[\S4.2.2]{fontaine:representations_semi-stables}, then $D_{K_v}:=(\Kbar_v\otimes_{\bQ_p^\nr}D)^{G_v}$ is a filtered $K_v$-vector space for which the canonical map
	\[
	\Kbar_v\otimes_{K_v}D_{K_v}\to\Kbar_v\otimes_{\bQ_p^\nr}D
	\]
	induced from the inclusion $D_{K_v}\hookrightarrow\Kbar_v\otimes_{\bQ_p^\nr}D$ is a filtered isomorphism (by Galois descent). Taking~$c_\BO$ to be the inverse of this isomorphism yields a filtered discrete $(\varphi,N,G_v)$-module $(D,D_{K_v},c_\BO)$ in the sense of Definition~\ref{def:discretephiNGvmodule}.
\end{rmk}

\begin{ex}
	\alex{24/3}{Insert a discussion of crystalline cohomology here: $D:=\bQ_p^\nr\otimes_{K_0}\rH^i_\cris$, $D_{K_v}:=\rH^i_\deR$ and $c_\BO=$ Bloch--Ogus isomorphism defines a filtered discrete $(\varphi,N,G_v)$-module}
\end{ex}

\alex{24/3}{We need to update the later parts of this section to match this new definition of $(\varphi,N,G_v)$-modules}

To assign a filtered discrete $(\varphi,N,G_v)$-module to a de Rham representation~$V$, Fontaine introduces a second period ring~$\sB_\st$ \cite[\S3.1]{fontaine:corps_des_periodes}, which is a~$\bQ_p^\nr$-algebra with an action of~$G_v$ extending the natural action on~$\bQ_p^\nr$. For a representation~$V$ of~$G_v$, one defines
\[
\sD_\pst(V):=\varinjlim_w\left(\sB_\st\otimes_{\bQ_p}V\right)^{G_w} \,,
\]
where the colimit is taken over open subgroups $G_w\leq G_v$ \cite[\S5.6.4]{fontaine:representations_semi-stables}. This is a $\bQ_p^\nr$-vector space of dimension at most $\dim_{\bQ_p}(V)$ \cite[Th\'eor\`eme~5.6.7(i)]{fontaine:representations_semi-stables}, and carries a natural action of~$G_v$ with open point-stabilisers, namely the restriction of the action on $\sB_\st\otimes_{\bQ_p}V$.

The period ring $\sB_\st$ carries a $G_v$-equivariant injective Frobenius \cite[\S3.2.1]{fontaine:corps_des_periodes} and monodromy operator \cite[\S3.2.2]{fontaine:corps_des_periodes} satisfying $N\circ\varphi=p\cdot\varphi\circ N$. These
induce on $\sD_\pst(V)$ the structure of a discrete $(\varphi,N,G_v)$-module for every representation~$V$ of~$G_v$. Moreover, $\sB_\st$ is a $\bQ_p^\nr$-subalgebra\footnote{Usually, one adopts the point of view that the embedding $\sB_\st\hookrightarrow\sB_\deR$ is non-canonical, depending on a choice of $p$-adic logarithm. However, we shall adopt the point of view of \cite{shimizu:p-adic_monodromy}, identifying $\sB_\st$ with its image under this embedding, which is independent of the choice of $p$-adic logarithm.} of~$\sB_\deR$, so there is for every $G_v$-representation~$V$ a natural $K_v$-linear map
\[
\sD_\pst(V)_{K_v}\to\sD_\deR(V),
\]
which is an isomorphism when~$V$ is de Rham \cite[Th\'eor\`eme~5.6.7(ii)]{fontaine:representations_semi-stables}\cite[Th\'eor\`eme~0.7]{berger:representations_p-adiques}. In this way, the Hodge filtration on~$\sD_\deR(V)$ induces a corresponding filtration on $\sD_\pst(V)_{K_v}$, and hence induces on $\sD_\pst(V)$ the structure of a filtered discrete $(\varphi,N,G_v)$-module.

Although it is not strictly necessary in what follows, we note that the theory of filtered $(\varphi,N,G_v)$-modules suffices to capture the category of de Rham representations.

\begin{thm}[{\cite[Th\'eor\`eme~5.6.7(v)]{fontaine:representations_semi-stables}}, {\cite[Th\'eor\`eme~0.7]{berger:representations_p-adiques}}]
The assignment 
\[
V\mapsto\sD_\pst(V)
\]
gives a fully faithful $\otimes$-functor
\[
\sD_\pst\colon \Rep_{\bQ_p}^\deR(G_v)\hookrightarrow\MF(\varphi,N,G_v) \,,
\]
where $\MF(\varphi,N,G_v)$ denotes the $\otimes$-category of filtered discrete $(\varphi,N,G_v)$-modules.
\end{thm}

\subsubsection{Automorphisms of discrete $(\varphi,N,G_v)$-modules}

In the argument of Lawrence--Venkatesh, it will be important at one point to put upper bounds on the dimensions of automorphism groups of $(\varphi,N,G_v)$-modules.

\begin{defi}
\leavevmode
\begin{enumerate}
	\item Let $D$ be a discrete $(\varphi,N,G_v)$-module. An \emph{automorphism} of $D$ is a $\bQ_p^\nr$-linear automorphism of $D$ which commutes with the actions of $\varphi$, $N$ and $G_v$. More generally, if $R$ is a $\bQ_p$-algebra, an \emph{$R$-linear automorphism} of $D$ is a $R\otimes_{\bQ_p}\bQ_p^\nr$-linear automorphism of $R\otimes_{\bQ_p}D$ which commutes with the actions of $1\otimes\varphi$, $1\otimes N$ and the action of~$G_v$ on~$D$. We will see shortly that the functor
\[
\uAut(D)\colon\{\text{$\bQ_p$-algebras}\}\rightarrow \{\text{groups}\} %\Groups
\]
sending a $\bQ_p$-algebra $R$ to the group of $R$-linear automorphisms of $D$ is representable by an affine algebraic group over $\bQ_p$, which we also call $\uAut(D)$.
	\item If $(D,\omega)$ is a symplectic discrete $(\varphi,N,G_v)$-module, then we define $\uAut(D,\omega)$ to be the closed algebraic subgroup of $\uAut(D)$ consisting of those automorphisms which preserve the pairing $\omega$.
\end{enumerate}
\end{defi}

\begin{prop}\label{prop:dim_of_aut}
\leavevmode
\begin{enumerate}
	\item\label{proppart:dim_of_aut_basic} Let $D$ be a discrete $(\varphi,N,G_v)$-module of dimension $d$. Then $\uAut(D)$ is a closed $\bQ_p$-algebraic subgroup of $\Res^{K_v}_{\bQ_p}\uAut_{K_v}(D_{K_v})$ of $\bQ_p$-dimension $\leq d^2$.
	\item\label{proppart:dim_of_aut_symplectic} Let $(D,\omega)$ be a symplectic discrete $(\varphi,N,G_v)$-module of rank $2d$. Then $\uAut(D,\omega)$ is a closed $\bQ_p$-algebraic subgroup of $\Res^{K_v}_{\bQ_p}\uAut_{K_v}(D_{K_v},\omega_{K_v})$ of $\bQ_p$-dimension $\leq d(2d+1)$.
\end{enumerate}
\begin{proof}
\eqref{proppart:dim_of_aut_basic} If $\psi$ is an endomorphism of $D$, then by applying the functor $(-)_{K_v}=(\Kbar_v\otimes_{\bQ_p^\nr}-)^{G_v}$ we obtain a $K_v$-linear endomorphism $\psi_{K_v}$ of $D_{K_v}$. This construction provides a morphism of not-necessarily-commutative $\bQ_p$-algebras
\[
\End(D)\rightarrow\End_{K_v}(D_{K_v})\,.
\]
This is easily seen to be injective, for, if $\psi_{K_v}=0$, then $1\otimes\psi$ acts as zero on $\Kbar_v\otimes_{\bQ_p^\nr}D=\Kbar_v\otimes_{K_v}D_{K_v}$, and hence $\psi=0$ already.

Now $\uAut(D)$ is the functor
\[
R\mapsto(R\otimes_{\bQ_p}\End(D))^\times
\]
and $\Res^{K_v}_{\bQ_p}\uAut_{K_v}(D_{K_v})$ is the functor
\[
R\mapsto(R\otimes_{\bQ_p}\End_{K_v}(D_{K_v}))^\times\,,
\]
so that the above construction yields an injective morphism of functors 
\begin{equation}
\label{eq:closedimmersionAutinAut}
\uAut(D)\hookrightarrow\Res^{K_v}_{\bQ_p}\uAut_{K_v}(D_{K_v}).
\end{equation}
Since this is induced by an injective morphism of not-necessarily-commutative, but finite dimensional $\bQ_p$-algebras, this is a closed immersion of algebraic groups.

To establish the dimension inequality, we will show that the morphism 
\begin{equation}
\label{eq:closedimmersionKvlinearAut}
\uAut(D)_{K_v}\rightarrow\uAut_{K_v}(D_{K_v})
\end{equation}
corresponding to the closed immersion \eqref{eq:closedimmersionAutinAut}
%$\uAut(D)\hookrightarrow\Res^{K_v}_{\bQ_p}\uAut_{K_v}(D_{K_v})$ 
under the base-change--Weil-restriction adjunction is also a closed immersion of affine algebraic groups over $K_v$. This shows that 
\[
\dim_{\bQ_p}\uAut(D) =   \dim_{K_v}  \uAut(D)_{K_v}   \leq\dim_{K_v}\uAut_{K_v}(D_{K_v}) = \dim \GL_d = d^2
\]
as claimed.

To see that this map is a closed immersion, it suffices to prove that the morphism
\begin{equation}
\label{eq:KvlinearmapofEndos}
K_v\otimes_{\bQ_p}\End(D) \rightarrow \End_{K_v}(D_{K_v})
\end{equation}
of not-necessarily-commutative, but finite dimensional $K_v$-algebras is also injective. Suppose that $\psi_1,\dots,\psi_k$ are $\bQ_p$-linearly independent endomorphisms of $D$ and $\lambda_1,\dots,\lambda_k$ are elements of $K_v$ such that $\psi:=\sum_i\lambda_i\otimes\psi_i$ restricts to the zero endomorphism of $D_{K_v}=(\Kbar_v\otimes_{\bQ_p^\nr}D)^{G_v}$. Then $\psi$ acts as zero on $\Kbar_v\otimes_{\bQ_p^\nr}D$. Since each $\psi_i$ commutes with the $G_v$-action, we know that for all $\sigma\in G_v$ and all $\alpha\in K_v$
\[
\sigma(\alpha\psi)=\sum_i\sigma(\alpha\lambda_i)\otimes\psi_i
\]
also acts as zero on $\Kbar_v\otimes_{\bQ_p^\nr}D$.  This then implies that 
\[
\sum_i\tr_{K_v/\bQ_p}(\alpha\lambda_i)\otimes\psi_i=0.
\]
The $\psi_i$ being $\bQ_p$-linear independent implies that $\tr_{K_v/\bQ_p}(\alpha\lambda_i)=0$ for all $\alpha\in K_v$ and all $i$. Non-degeneracy of the trace pairing shows $\lambda_i=0$ for all $i$ and so $\psi=0$. Thus the map \eqref{eq:KvlinearmapofEndos} 
%$K_v\otimes_{\bQ_p}\End(D)\rightarrow\End_{K_v}(D_{K_v})$ 
is injective as claimed.

\eqref{proppart:dim_of_aut_symplectic} The closed immersions \eqref{eq:closedimmersionAutinAut}
%$\uAut(D)\hookrightarrow\Res^{K_v}_{\bQ_p}\uAut_{K_v}(D_{K_v})$ 
and \eqref{eq:closedimmersionKvlinearAut}
%$\uAut(D)_{K_v}\hookrightarrow\uAut_{K_v}(D_{K_v})$ 
constructed in the first part restrict to closed immersions 
\[
\uAut(D,\omega)\hookrightarrow\Res^{K_v}_{\bQ_p}\uAut_{K_v}(D_{K_v},\omega_{K_v}) \quad \text{ and } \quad \uAut(D,\omega)_{K_v}\hookrightarrow\uAut_{K_v}(D_{K_v},\omega_{K_v}).
\]
The result follows in view of $\dim \Sp_{2d} = d(2d+1)$.
\end{proof}
\end{prop}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Self-conjugate places}\label{ss:friendly}

In the Lawrence--Venkatesh method, it is necessary to work with places~$v$ of~$K$ which satisfy a particular technical assumption, known as \emph{friendliness} \cite[Definition~2.7]{LV}. For our purposes, it suffices to work with a somewhat weaker notion.

\begin{defi}[Self-conjugate places, cf.\ {\cite[Definition~2.7]{LV}}]\label{def:friendly}
%We say that two $p$-adic places~$v$ and~$\bar v$ of~$K$ are \emph{conjugate} just when their restrictions to every CM subfield~$E$ of~$K$ are conjugate under the complex conjugation on~$E$. We say that a place $v$ is \emph{self-conjugate} if it is conjugate to itself.
We say that a finite place~$v$ of a number field~$K$ is \emph{self-conjugate} just when its restriction to every CM subfield~$E\subseteq K$ is invariant under the conjugation on~$E$.
\end{defi}

\begin{rmk}
(1) If~$K$ contains no CM subfield, then every finite place is self-conjugate. 

(2) If~$K$ contains a CM subfield, then it has a maximal CM subfield~$E$, and a finite place~$v$ of~$K$ is self-conjugate if and only if its restriction to~$E$ is invariant under the conjugation on~$E$.

%If~$K$ contains no CM subfield, then every place is self-conjugate. If instead~$K$ contains a CM subfield, then it has a maximal CM subfield~$E$; a place~$v$ is self-conjugate if and only if its restriction to the maximal totally real subfield~$E^+$ of~$E$ is inert or ramified in~$E$.
(3) The \emph{friendly places} of \cite[Definition~2.7]{LV} are exactly the self-conjugate places which are unramified over~$\bQ$.
\end{rmk}

The property of self-conjugate places~$v$ which is relevant in the Lawrence--Venkatesh argument is that if~$V$ is a representation of~$G_K$ which is pure of some weight, then the average Hodge--Tate weight of~$V|_{G_v}$ is determined by the weight of~$V$. To prove this, one first deals with the case of $1$-dimensional representations.

\begin{prop}[cf.\ {\cite[Lemma~2.8]{LV}}]\label{prop:friendly_characters}
Let $v$ be a self-conjugate $p$-adic place of $K$. Suppose that $\chi\colon \Gal_K\rightarrow\bQ_p^\times$ is a $p$-adic character  such that:
\begin{enumerate}[label=(\roman*)]
	\item $\chi$ is unramified and pure of weight~$n\in\bZ$ outside a finite set of places of~$K$, and
	\item $\chi$ is Hodge--Tate at all places over~$p$, and has Hodge--Tate weight\footnote{The \emph{Hodge--Tate weights} of a representation $V$ of $G_v$ are the integers $r$ such that $(\bC_p(r)\otimes_{\bQ_p}V)^{G_v}\neq0$, where the $G_v$ action on $\bC_p(r)$ is the $r$th Tate twist of the natural action on $\bC_p$. The \emph{multiplicity} of a Hodge--Tate weight $r$ is the $\bQ_p$-dimension of $(\bC_p(r)\otimes_{\bQ_p}V)^{G_v}$. The total number of Hodge--Tate weights, counting multiplicity, is at most $\dim_{\bQ_p}V$, with equality if and only if $V$ is Hodge--Tate.} $r$ at~$v$.
\end{enumerate}
Then $r=n/2$ (and $n$ is even).
\begin{proof}
The proof of \cite[Lemma~2.8]{LV} works verbatim. The assumption that~$v$ is unramified over~$\bQ$ is not used in the proof.
\end{proof}
\end{prop}

\jakob{17.12.2020}{I am confused by the proof of  \cite[Lemma~2.8]{LV} and for a good reason as the next remark shows. Therefore, I think, we should give a full proof and not state that this works verbatim.}

\begin{rmk}
\cite[Lemma~2.8]{LV} asserts a stronger structural result: that $\chi|_{G_v}$ is, up to a finite-order character, a power of the cyclotomic character. The proof, however, only seems to establish this for the restriction to the inertia group~$I_v$. The argument in \cite{LV} shows that the $v$-component~$\eta_v$ of the Hecke character $\eta\colon\bA_K^\times/K^\times\to\bQ_p^\times$ corresponding to~$\chi$ agrees, in a neighbourhood of $1\in K_v^\times$, with an algebraic Hecke character $\eta_v^\alg\colon\Res^{K_v}_{\bQ_p}\bG_{m,K_v}\to\bG_{m,\bQ_p}$, which is shown to be the $n/2$th power of the norm character $\Res^{K_v}_{\bQ_p}\bG_{m,K_v}\to\bG_{m,\bQ_p}$. From this, it is asserted that~$\eta_v$ is, up to a finite-order character, the $n/2$th power of the norm character~$K_v^\times\to\bQ_p^\times$, and hence that $\chi|_{G_v}$ is, up to a finite-order character, a power of the cyclotomic character. This does not in fact follow, since open subgroups of~$K_v^\times$ are not finite index. One can only deduce this for the restriction $\eta_v|_{\cO_v^\times}$, and hence one only obtains that $\chi|_{I_v}$ is, up to a finite-order character, a power of the cyclotomic character. Since the Hodge--Tate weights of a Hodge--Tate character depend only on its restriction to inertia \cite[Theorem~III.A5.2]{serre:reps_and_elliptic_curves}, this still suffices to prove the assertion on Hodge--Tate weights.
\end{rmk}

%\begin{prop}[cf.\ {\cite[Lemma~2.8]{LV}}]\label{prop:friendly_characters}
%Let $v$ and $\bar v$ be conjugate $p$-adic places of $K$. Suppose that $\chi\colon G_K\rightarrow\bQ_p^\times$ is a $p$-adic character of $G_K$ such that:
%\begin{itemize}
%	\item $\chi$ is unramified and pure of weight~$n\in\bZ$ outside a finite set of places of~$K$; and
%	\item $\chi$ is Hodge--Tate at all places over~$p$, and has Hodge--Tate weights\footnote{The \emph{Hodge--Tate weights} of a representation $V$ of $G_v$ are the integers $r$ such that $(\bC_p(r)\otimes_{\bQ_p}V)^{G_v}\neq0$, where the $G_v$ action on $\bC_p(r)$ is the $r$th Tate twist of the natural action on $\bC_p$. The \emph{multiplicity} of a Hodge--Tate weight $r$ is the $\bQ_p$-dimension of $(\bC_p(r)\otimes_{\bQ_p}V)^{G_v}$. The total number of Hodge--Tate weights, counting multiplicity, is at most $\dim_{\bQ_p}V$, with equality if and only if $V$ is Hodge--Tate.} $r$ and $\bar r$ at $v$ and $\bar v$, respectively.
%\end{itemize}
%Then $r+\bar r=n$.

%In particular, if $v=\bar v$ is self-conjugate, then $r=n/2$ (and $n$ is even).
%\begin{proof}
%By global class field theory, $\chi$ corresponds to a continuous idele class character
%\[
%\eta\colon\bA_K^\times\rightarrow\bQ_p^\times
%\]
%which is trivial on $K^\times$. We write
%\[
%\eta_p\colon(K\otimes_\bQ\bQ_p)^\times\rightarrow\bQ_p^\times
%\]
%for the component of $\eta$ at places above $p$. By a theorem of Tate \cite[Theorem~on~p.III-7]{serre:reps_and_elliptic_curves}, the Hodge--Tate condition implies that $\eta_p$ agrees, in a neighbourhood of $1\in(K\otimes_\bQ\bQ_p)^\times$, with an algebraic character
%\[
%\eta_p^\alg\colon\bT^{(K)}_{\bQ_p}\rightarrow\bG_{m,\bQ_p}\,,
%\]
%where $\bT^{(K)}:=\Res^K_\bQ\bG_{m,K}$ is the algebraic torus associated to $K^\times$ \cite[\S II.1.1]{serre:reps_and_elliptic_curves}. The fact that $\eta$ is finitely ramified implies that $\eta_p$, and hence $\eta_p^\alg$, vanishes on a finite-index subgroup of the units $\cO_K^\times$. It follows that $\eta_p^\alg$ factors through $\bS^{(K)}_{\bQ_p}$ where $\bS^{(K)}$ is the \emph{Serre torus}, i.e.\ the quotient of $\bT^{(K)}$ by the identity component of the Zariski-closure of $\cO_K^\times\subseteq K^\times=\bT(\bQ)$.

%\smallskip
%\textbf{Case 1:} Suppose firstly that $K$ contains no CM subfield. Then the norm map $\rN_{K/\bQ}\colon\bS^{(K)}\rightarrow\bG_{m,\bQ}$ is an isogeny \todo{?}, so, replacing $\chi$ by a power if necessary, we may assume that $\eta_p^\alg=\rN_{K/\bQ}^{n'/2}$ for some even integer $n'$. It remains to show that $r=n'/2$ and $n=n'$.

%For the first of these, the fact that $\chi$ is Hodge--Tate of weight~$r$ at~$v$ implies that $\chi$ agrees with the $-r$th power of the cyclotomic character on an open subgroup of the inertia group $I_v$ \cite[Theorem~III.A5.2]{serre:reps_and_elliptic_curves}. This in turn implies that the restriction of $\eta_p^\alg$ to the subtorus $\Res^{K_v}_{\bQ_p}\bG_{m,K_v}\subseteq\bT^{(K)}_{\bQ_p}$ is equal to the $r$th power of the norm map $\rN_{K_v/\bQ_p}\colon\Res^{K_v}_{\bQ_p}\bG_{m,K_v}\rightarrow\bG_{m,\bQ_p}$. Since $\eta_p^\alg$ is the $n'/2$th power of the norm map, this implies that $r=n'/2$ as claimed.

%For the second of these, we may choose a finite set $T$ of places of $K$, containing all places dividing~$p\infty$, such that $\chi$ is pure of weight $n$ outside $T$. This implies that for all $\lambda\in K^\times$ which is sufficiently close to $1$ at all places in $T$, the value $\eta_p^\alg(\lambda)=\eta_p(\lambda)\in\bQ_p^\times$ is an algebraic number such that $|\iota(\eta_p^\alg(\lambda))|=\rN_{K/\bQ}(\lambda)^{n/2}$ for all complex embeddings $\iota\colon\bQ_p\hookrightarrow\bC$. Since $\eta_p^\alg(\lambda)=\rN_{K/\bQ}(\lambda)^{n'/2}$, this implies that $n=n'$ as claimed.

%\smallskip
%\textbf{Case 2:} Suppose instead that $K$ contains a CM subfield, and let $E$ be its maximal CM subfield. In this case, the norm map $\rN_{K/E}\colon\bS^{(K)}\rightarrow\bS^{(E)}$ is an isogeny \cite{?}, so, replacing $\chi$ with a power if necessary, we may assume that $\eta_p^\alg$ factors through $\bS^{(E)}_{\bQ_p}$.

%Now $E$ carries a complex conjugation, which acts also on $\bS^{(E)}$. Since $\eta_p^\alg$ factors uniquely through the norm map to $\bS^{(E)}_{\bQ_p}$, we may form the conjugate character $\bar\eta_p^\alg$ by composing $\eta_p^\alg$ with the conjugation on $\bS^{(E)}_{\bQ_p}$. Then $\eta_p^\alg\bar\eta_p^\alg$ factors through a conjugation-invariant character of $\bS^{(E)}_{\bQ_p}$. But the norm map $\rN_{E/E^+}\colon\bS^{(E)}\rightarrow\bS^{(E^+)}$ from $E$ to its maximal totally real subfield $E^+$ induces an isogeny from the conjugation-coinvariants of $\bS^{(E)}$ to $\bS^{(E^+)}$ \cite{obvious?}, and as above $\bS^{(E^+)}$ is isogenous to $\bG_{m,\bQ}$ via the norm map from $E^+$ to $\bQ$. Thus, replacing $\chi$ with a further power if necessary, we may assume that $\eta_p^\alg\bar\eta_p^\alg=\rN_{K/\bQ}^{n'}$ for some integer $n'$. It suffices to prove that $n'=r+\bar r$ and $n'=n$.

%For the first of these, we note as above that the restriction of $\eta_p^\alg$ to $\Res^{K_v}_{\bQ_p}\bG_{m,K_v}\subseteq\bT^{(K)}_{\bQ_p}$ is the $r$th power of the norm map $\rN_{K_v/\bQ_p}$. Similarly, the restriction of the conjugate character $\bar\eta_p^\alg$ to $\Res^{K_v}_{\bQ_p}\bG_{m,K_v}\subseteq\bT^{(K)}_{\bQ_p}$ is the $\bar r$th power of the norm map $\rN_{K_v/\bQ_p}$. Since $\eta_p^\alg\bar\eta_p^\alg$ is the $n'$th power of the norm map, this implies that $r+\bar r=n'$ as claimed.

%For the second of these, we note as above that for every $\lambda\in K^\times$ which is sufficiently close to $1$ at every place in $T$ we have that $|\iota(\eta_p^\alg(\lambda))|=\rN_{K/\bQ}(\lambda)^{n/2}$ for every complex embedding $\iota\colon\bQ_p\hookrightarrow\bC$. Similarly, enlarging $T$ if necessary, we have $|\iota(\bar\eta_p^\alg(\lambda))|=\rN_{E/\bQ}\left(\overline{\rN_{K/E}(\lambda)}\right)^{n/2}=\rN_{K/\bQ}(\lambda)^{n/2}$ for every complex embedding $\iota$. Since $\eta_p^\alg(\lambda)\cdot\bar\eta_p^\alg(\lambda)=\rN_{K/\bQ}(\lambda)^{n'}$, this implies that $n=n'$ as claimed.
%\end{proof}
%\end{prop}

\begin{cor}[cf.\ {\cite[Lemmas~2.9~and~2.10]{LV}}]\label{cor:friendly_representations}
Let $L/K$ be a finite extension and~$V$ a representation of~$\Gal_L$ which is de Rham at all places of~$L$ above~$p$ and unramified and pure of weight $n\in\bZ$ outside a finite set of places of~$L$. Let~$v$ be a self-conjugate place of~$K$ above~$p$. Then
\[
\sum_{w\mid v}[L_w:K_v]\left(\sum_{i\in\bZ}i\dim_{L_w}\gr_{\rF}^i\sD_{\deR,w}(V)\right) = \frac{n\cdot[L:K]\cdot\dim_{\bQ_p}(V)}{2}\,,
\]
where the summation runs through places~$w$ of~$L$ dividing~$v$, the filtered $L_w$-vector space 
\[
\sD_{\deR,w}(V)=(\sB_\deR\otimes_{\bQ_p}V)^{G_w}
\]
is Fontaine's de Rham functor applied to the restriction of $V$ to a decomposition group at~$w$, and $\rF^\bullet$ is the Hodge filtration.
\begin{proof}
The induced representation $W = \Ind_{\Gal_L}^{\Gal_K}(V)$ is again unramified outside a finite set of places of $K$, and it is pure of the same weight $n$ (weights can be read off after restriction to open subgroups of $\Gal_K$, and for a suitable such the induced representation will decompose as a direct sum of conjugates of the restriction of $V$). 

For a place $w \mid v$ above $p$, the local induced representation $W_w = \Ind_{G_w}^{G_v}(V)$ has
\[
\sD_{\deR,w}(V) = (\sB_\deR\otimes_{\bQ_p}V)^{G_w} = (\sB_\deR\otimes_{\bQ_p} W_w)^{G_v} = \sD_{\deR,v}(W_w)
\]
as filtered $K_v$-vector spaces. Since $W = \bigoplus_{w \mid v} W_w$ as $G_v$-representation, 
%\[
%W|_{G_v} = \bigoplus_{w \mid v} \Ind_{G_w}^{G_v}(V|_{G_w})
%\]
the representation $W$ is also de Rham at all places above $p$. The Hodge-Tate weight $i$ occurs with multiplicity 
\[
\dim_{K_v} \Big(\gr_{\rF}^i\sD_{\deR,v}(W)\Big) 
= \sum_{w \mid v} [L_w:K_v] \cdot \dim_{L_w} \Big(\gr_{\rF}^i\sD_{\deR,w}(V)\Big).
\]

We now apply Proposition~\ref{prop:friendly_characters} to the character $\chi = \det(W)$. 
%\det\left(\Ind_{\Gal_L}^{\Gal_K}V\right)$. 
The character $\chi$ is unramified and pure of weight $n\cdot[L:K]\cdot\dim_{\bQ_p}(V)$ outside a finite set of places of $K$. It is also de Rham at places above $p$ and the Hodge-Tate weight at $v$ is 
\[
\sum_{i \in \bZ}  i\dim_{K_v}  \Big(\gr_{\rF}^i\sD_{\deR,v}(W)\Big) = \sum_{w\mid v}[L_w:K_v]\left(\sum_{i\in\bZ}i\dim_{L_w}  \Big(\gr_{\rF}^i\sD_{\deR,w}(V)\Big)\right).  \qedhere
\]
\end{proof}
\end{cor}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Preliminaries: families of Galois representations and $v$-adic period maps}

\alex{23/4}{Given how long this section is, do you think there's an argument that we should move the stuff about getting finiteness from period maps, comparison with~$\bC$ and monodromy calculations to its own section?}

The method of Lawrence--Venkatesh revolves around the study of families of Galois representations arising from smooth proper morphisms $\pi\colon X\to Y$ of smooth 
%
%\jakob{12.02.2021}{Do we need $Y$ to be smooth?}
%\alex{18.02.2021}{I believe so -- when we do all this relative $p$-adic Hodge theory, we want to know that every $K_v$-point of~$Y^\an$ has an admissible neighbourhood isomorphic to a unit disc.}
%
$K$-varieties. In this section, we collect various results about such families of Galois representations which will be used in the sequel.

The structure of this section is as follows. In \S\ref{ss:period_maps}, we recall the definition of the period map(s) associated to a smooth proper morphism $\pi\colon X\to Y$ of smooth $K_v$-varieties, and state the main result of this section (Theorem~\ref{thm:period_maps_control_reps} and Corollary~\ref{cor:period_maps_control_reps}): that these period maps describe how the \'etale cohomology of the fibres~$X_y$ varies locally for~$y\in Y(K_v)$. In \S\ref{ss:period_maps_complex}, we discuss how the image of the $v$-adic period map can be controlled using monodromy over the complex numbers, and give a criterion for showing that a subset of~$Y(K_v)$ is finite when~$Y$ is a smooth projective curve. This is all the background material that is required for the proof of the Mordell Conjecture via the Lawrence--Venkatesh method.

In \S\ref{ss:local_systems}, we give the formal definition of a ``family of Galois representations'', namely a $\bQ_p$-local system (a.k.a.\ lisse sheaf). This is used only implicitly in~\cite{LV}, but will be necessary in the proof of our main theorem \todo{ref}. The final section~\S\ref{ss:relative_p-adic_hodge} is devoted to proving Theorem~\ref{thm:period_maps_control_reps}, that period maps describe variations of Galois representations. It is here that our approach differs most from that in~\cite{LV}: in the absence of good reduction hypotheses, we cannot use the theory of crystalline cohomology as a bridge between \'etale and de Rham cohomology, and are forced instead to use tools from relative $p$-adic Hodge theory, as developed by Scholze~\cite{scholze:relative_p-adic_hodge_theory} and Shimizu~\cite{shimizu:p-adic_monodromy}.

\subsection{Period maps}\label{ss:period_maps}

Suppose that~$Y$ is a smooth $K_v$-variety, and let~$(V,\nabla)$ be a vector bundle\footnote{A vector bundle on a rigid-analytic space~$S$ over~$K_v$ is an~$\cO_S$-module which is locally finite free. Here, the topology can equivalently be taken to be the analytic, \'etale or pro-\'etale topology \cite[Lemma~7.3]{scholze:relative_p-adic_hodge_theory}.} with flat\footnote{In our applications, we will only be working over one-dimensional bases, where every rigid analytic connection is automatically flat.} connection on the rigid analytification~$Y^\an$ (e.g.\ the analytification of an algebraic vector bundle on~$Y$ with flat connection). Suppose that~$\Nbd_{y_0}\subseteq Y^\an$ is an admissible open neighbourhood of a point $y_0\in Y(K_v)$, such that $\rH^0_\deR(\Nbd_{y_0}/K_v)=K_v$; for instance, $\Nbd_{y_0}$ could be isomorphic to a closed polydisc or a closed polyannulus. We say that~$(V,\nabla)$ has a \emph{full basis of horizontal sections} over~$\Nbd_{y_0}$ just when $(V,\nabla)|_{\Nbd_{y_0}}\simeq(\cO_{\Nbd_{y_0}},\rd)^{\oplus m}$ for some~$m$. The vector bundle $(V,\nabla)$ always admits a full basis of horizontal sections over a sufficiently small neighbourhood of~$y_0$ (Proposition~\ref{prop:explicit_parallel_transport})\todo{?}.

When~$(V,\nabla)$ has a full basis of horizontal sections over~$\Nbd_{y_0}$, then there is a \emph{canonical} isomorphism
\[
T^\nabla_{y_0}\colon(\cO_{\Nbd_{y_0}}\otimes_{K_v}V_{y_0},\rd\otimes1)\xrightarrow\sim(V,\nabla)|_{\Nbd_{y_0}} \,,
\]
characterised by the fact that the fibre of~$T^\nabla_{y_0}$ at~$y_0$ is the identity map. The fibre of $T^\nabla_{y_0}$ at another point $y\in\Nbd_{y_0}(K_v)$ is an isomorphism $T^\nabla_{y_0,y}\colon V_{y_0}\xrightarrow\sim V_y$ from the fibre over~$y_0$ to the fibre over~$y$, known as the \emph{parallel transport} map.

Using parallel transport, one can define the period map associated to a filtered vector bundle with flat connection.

\alex{24/3}{We said that we wanted to redefine the flag variety~$\dG_{y_0}$ to be the one representing the functor taking a scheme~$S$ to the set of isomorphism classes of pairs $(\dE,c)$ of a filtered vector bundle~$\dE$ on~$S$ and an isomorphism $c\colon\dE\xrightarrow\sim \cO_S\otimes_{K_v}V_{y_0}$. This is the same as the flag variety, but presented slightly differently. I may have to think a bit more about whether this is desirable, in light of some of the calculations we do later with filtrations}

\begin{defi}\label{def:period_maps}
Let~$Y$ be a smooth variety over~$K_v$, and let $(V,\nabla)$ be a vector bundle with flat connection on~$Y^\an$ endowed with an exhaustive, separated descending filtration $\dots\geq\rF^{-1}V\geq\rF^0V\geq\rF^{1}V\geq\dots$ (not necessarily stable\footnote{In practice, the filtrations appearing will all satisfy Griffiths transversality with respect to the connection, but this is not necessary to define the period map.} under the connection~$\nabla$) whose graded pieces are all vector bundles.

For $y_0\in Y(K_v)$, we define the \emph{period domain} to be the flag variety~$\dG_{y_0}$ parametrising filtrations on~$V_{y_0}$ with the same dimension data as~$\rF^\bullet V_{y_0}$. If~$\Nbd_{y_0}\subseteq Y^\an$ is an admissible open neighbourhood of~$y_0$ such that~$\rH^0_\deR(\Nbd_{y_0}/K_v)=K_v$ and~$(V,\nabla)$ has a full basis of horizontal sections over~$\Nbd_{y_0}$, then we define the ($v$-adic) \emph{period map} to be the $K_v$-analytic map
\[
\Phi_{y_0}\colon\Nbd_{y_0}\to\dG_{y_0}^\an
\]
classifying the filtration on $\cO_{\Nbd_{y_0}}\otimes_{K_v}V_{y_0}$ given by pulling back the filtration~$\rF^\bullet$ along the parallel transport map~$T_{y_0}^\nabla$.

Concretely, if $y\in\Nbd_{y_0}(K_v)$, then $\Phi_{y_0}(y)$ is the $K_v$-point of $\dG_{y_0}$ corresponding to the filtration on~$V_{y_0}$ given by pulling back the Hodge filtration on~$V_y$ along the parallel transport map $T^\nabla_{y_0,y}$.

%Concretely, if $y\in\Nbd_{y_0}(K_v)$, then $\Phi_{y_0}(y)$ is the class of the filtration~$T_{y_0,y}^{\nabla,*}(\rF^\bullet V_y)$, where $T_{y_0,y}^\nabla\colon V_{y_0}\xrightarrow\sim V_y$ is the parallel transport map.
\end{defi}

Implicitly in this description, we used the following description of the analytification of the flag variety~$\dG_{y_0}$.

\begin{prop}\label{prop:analytic_flag_variety}
Let~$V$ be a finite-dimensional~$K_v$-vector space, and let $(d_i)_{i\in\bZ}$ be non-negative integers summing to~$\dim_{K_v}V$. Let~$\dG/K_v$ denote the flag variety parametrising filtrations on~$V$ with dimension data $(d_i)_{i\in\bZ}$. Then the rigid analytification $\dG^\an$ represents the functor
\[
S\mapsto\{\text{filtrations $\rF^\bullet$ on $\cO_S\otimes_{K_v}V$ such that each $\gr_{\rF}^i(\cO_S\otimes_{K_v}V)$ is a vector bundle of rank $d_i$}\}
\]
from $K_v$-analytic spaces to sets.
\begin{proof}
The flag variety~$\dG$ represents the functor
\[
S\mapsto\{\text{filtrations $\rF^\bullet$ on $\cO_S\otimes_{K_v}V$ such that each $\gr_{\rF}^i(\cO_S\otimes_{K_v}V)$ is a vector bundle of rank $d_i$}\}
\]
from $K_v$-schemes to sets. By~\cite[Proposition~A.3.1]{conrad:analytification}, it follows that its analytification~$\dG^\an$ represents the functor
\[
A\mapsto\{\text{filtrations $\rF^\bullet$ on $A\otimes_{K_v}V$ such that each $\gr_{\rF}^i(A\otimes_{K_v}V)$ is finite projective of rank $d_i$}\}
\]
on strictly affinoid $K_v$-algebras~$A$. Using~\cite[Proposition~4.7.2]{fresnel-van_der_put:rigid_analytic_geometry}\footnote{Strictly speaking, \cite[Proposition~4.7.2]{fresnel-van_der_put:rigid_analytic_geometry} only asserts that there is a natural bijection between isomorphism classes of vector bundles on $\Sp(A)$ and finite projective $A$-modules. However, the proof shows the more precise result we need, that the functor $M\mapsto\widetilde M$ \cite[Definition~4.2.1]{fresnel-van_der_put:rigid_analytic_geometry} gives an equivalence of categories from finite projective $A$-modules to vector bundles on~$\Sp(A)$, with quasi-inverse the global sections functor.}, we see that the right-hand side is the set of filtrations of $\cO_{\Sp(A)}\otimes_{K_v}V$ whose graded pieces are vector bundles of the appropriate dimensions. Thus~$\dG^\an$ represents the claimed functor on affinoid analytic spaces, and hence in general by a gluing argument.
\end{proof}
\end{prop}

The importance of period maps is that they give a concrete description of how Galois representations vary in families. This is true in a great level of generality, but for our purposes, it suffices to consider only those families of Galois representations arising from smooth proper families of varieties. Consider a smooth proper morphism~$\pi\colon X\to Y$ of smooth $K_v$-varieties, and let~$\cH^i_\deR(X/Y)$ denote the $i$th relative de Rham cohomology of~$X$ over~$Y$ \todo{citation}. This is a vector bundle on~$Y$ endowed with a Hodge filtration~$\rF^\bullet$ and a flat Gauss--Manin connection~$\nabla$ \cite[Theorem~1]{katz-oda:relative_de_rham}. For any point~$y\in Y(K_v)$, the fibre of~$\cH^i_\deR(X/Y)^\an$ at~$y$ is canonically identified with the (algebraic) de Rham cohomology~$\rH^i_\deR(X_y/K_v)$ of the fibre~$X_y$, via the base change theorem for de Rham cohomology \todo{another citation}. If~$\Nbd\subseteq Y^\an$ is an admissible open subset, isomorphic to a closed polydisc, over which the analytification of~$\cH^i_\deR(X/Y)$ has a full basis of horizontal sections, and $y_0,y\in U(K_v)$, then by mild abuse of notation we will denote the composite
\[
\rH^i_\deR(X_{y_0}/K_v) \cong \cH^i_\deR(X/Y)^\an_{y_0} \xrightarrow[\sim]{T_{y_0,y}^\nabla} \cH^i_\deR(X/Y)^\an_y \cong \rH^i_\deR(X_y/K_v)
\]
also by~$T_{y_0,y}^\nabla$.

\begin{thm}\label{thm:period_maps_control_reps}
Let $\pi\colon X\to Y$ be a smooth proper morphism of smooth $K_v$-varieties, and let $\Nbd\subseteq Y^\an$ be an admissible open subset, isomorphic to a closed polydisc, over which $\cH^i_\deR(X/Y)^\an$ has a full basis of horizontal sections for the Gau\ss--Manin connection. Then for every $y_0,y\in\Nbd(K_v)$, there is a unique isomorphism
\[
T_{y_0,y}\colon\sD_\pst\left(\rH^i_\et(X_{y_0,\Kbar_v},\bQ_p)\right) \xrightarrow\sim \sD_\pst\left(\rH^i_\et(X_{y,\Kbar_v},\bQ_p)\right)
\]
of $(\varphi,N,G_v)$-modules making the diagram
\begin{center}
\begin{tikzcd}
	\Kbar_v\otimes_{\bQ_p^\nr}\sD_\pst\left(\rH^i_\et(X_{y_0,\Kbar_v},\bQ_p)\right) \arrow[r,"c_\BO","\sim"']\arrow[d,"T_{y_0,y}"',"\wr"] & \Kbar_v\otimes_{K_v}\sD_\deR\left(\rH^i_\et(X_{y_0,\Kbar_v},\bQ_p)\right) \arrow[r,"c_\deR","\sim"'] & \Kbar_v\otimes_{K_v}\rH^i_\deR(X_{y_0}/K_v) \arrow[d,"T_{y_0,y}^\nabla","\wr"'] \\
	\Kbar_v\otimes_{\bQ_p^\nr}\sD_\pst\left(\rH^i_\et(X_{y,\Kbar_v},\bQ_p)\right) \arrow[r,"c_\BO","\sim"'] & \Kbar_v\otimes_{K_v}\sD_\deR\left(\rH^i_\et(X_{y,\Kbar_v},\bQ_p)\right) \arrow[r,"c_\deR","\sim"'] & \Kbar_v\otimes_{K_v}\rH^i_\deR(X_y/K_v)
\end{tikzcd}
\end{center}
commute.
\begin{proof}
	See \S\ref{ss:relative_p-adic_hodge}, in particular~\S\ref{sss:proof_of_period_maps}.
\end{proof}
\end{thm}

\begin{rmk}
	There are several different definitions of the \'etale--de Rham comparison isomorphism~$c_\deR$ in the literature (e.g.\ \cite[Theorem~8.1]{faltings:crystalline_cohomology}, \cite[Theorem~A1]{tsuji:c_st_survey}), and the validity of Theorem~\ref{thm:period_maps_control_reps} depends, \emph{a priori}, on which definition is used. For the sake of clarity, the comparison isomorphism~$c_\deR$ for which we prove Theorem~\ref{thm:period_maps_control_reps} is the comparison isomorphism constructed by Scholze \cite[Corollary~1.8]{scholze:relative_p-adic_hodge_theory} in the setting of rigid analysis. Throughout this paper, all references to~$c_\deR$ should be taken to refer to this particular comparison isomorphism.
	
	Although many definitions of the comparison isomorphism are now known to agree by work of Nizio\l\ \cite{niziol:too_many_comparison_isos}, Scholze's is not among them. So it is not immediately obvious that Scholze's comparison isomorphism~$c_\deR$ satisfies the compatibilities of Theorem~\ref{thm:c_dr}\ref{thmpart:c_dr_compatibilities}; nonetheless, we will prove in \todo{write this part} that this is the case.
\end{rmk}

%\begin{thm}\label{thm:period_maps_control_reps}
%	Let $\pi\colon X\to Y$ be a smooth proper morphism of smooth $K_v$-varieties, and let $\Nbd\subseteq Y^\an$ be an admissible open subset, isomorphic to a closed polydisc, such that the analytification $\cH^i_\deR(X/Y)^\an$ of the relative de Rham cohomology has a full basis of horizontal sections over~$\Nbd$ for the Gau\ss--Manin connection \cite[Theorem~1]{katz-oda:relative_de_rham}. Then for every $y_0,y\in\Nbd(K_v)$, the parallel transport map
%	\[
%	T_{y_0,y}^\nabla\colon\rH^i_\deR(X_{y_0}/K_v) \xrightarrow\sim \rH^i_\deR(X_y/K_v)
%	\]
%	is induced by a (unique) isomorphism
%	\[
%	T_{y_0,y}^\nabla\colon\sD_\pst\left(\rH^i_\et(X_{y_0,\Kbar_v},\bQ_p)\right) \xrightarrow\sim \sD_\pst\left(\rH^i_\et(X_{y,\Kbar_v},\bQ_p)\right)
%	\]
%	of discrete $(\varphi,N,G_v)$-modules.

%\jakob{23.03.2021}{We should include in the statement the property that makes this parallel-transport map for the $\sD_\pst$-version unique.}
%\begin{proof}
%See \S\ref{ss:relative_p-adic_hodge}.
%\end{proof}
%\end{thm}
\alex{23/3}{I've commented out the old statement of the theorem and remark here}

%\begin{rmk}
%Implicit in the statement of Theorem~\ref{thm:period_maps_control_reps} is an isomorphism $\sD_\pst(\rH^i_\et(X_{y,\Kbar_v},\bQ_p))_{K_v}\cong\rH^i_\deR(X_y/\bQ_p)$ for every $y\in Y(K_v)$, for which we take the composite
%\[
%\sD_\pst(\rH^i_\et(X_{y,\Kbar_v},\bQ_p))_{K_v}\cong\sD_\deR(\rH^i_\et(X_{y,\Kbar_v},\bQ_p))\xrightarrow[\sim]{c_\deR}\rH^i_\deR(X_y/\bQ_p) \,,
%\]
%where the first isomorphism is induced from the inclusion $\sB_\st\hookrightarrow\sB_\deR$, and $c_\deR$ is the de Rham comparison isomorphism.

%Technically, there is a potential source of ambiguity in that, while several authors have constructed comparison isomorphisms (e.g.\ \cite[Theorem~8.1]{faltings:crystalline_cohomology}, \cite[Theorem~A1]{tsuji:c_st_survey}), it is not \emph{a priori} clear that these comparison isomorphisms are the same as one another. Although many of these comparison isomorphisms are now known to agree by work of Nizio\l\ \cite{niziol:too_many_comparison_isos}, the comparison isomorphism proven by Scholze in \cite[Corollary~1.8]{scholze:relative_p-adic_hodge_theory} is not among them.

%So, for clarity, the comparison isomorphism $c_\deR$ we take above is that constructed by Scholze (see \todo{ref}). We will prove in \todo{do it} that Scholze's comparison isomorphism obeys all the same compatibilities as Tsuji's.
%\end{rmk}

Theorem~\ref{thm:period_maps_control_reps} admits a useful rephrasing in terms of period maps.

\begin{cor}[Period maps control variation of local Galois representations]\label{cor:period_maps_control_reps}
Let $\pi\colon X\to Y$ be a smooth proper morphism of smooth $K_v$-varieties, let $y_0\in Y(K_v)$ be a $K_v$-rational point, and let $\Nbd_{y_0}\subseteq Y^\an$ be an admissible open neighbourhood of~$y_0$, isomorphic to a closed polydisc, over which $\cH^i_\deR(X/Y)^\an$ has a full basis of horizontal sections. Then for all $y\in\Nbd_{y_0}(K_v)$, we have an isomorphism
\[
\left(\sD_\pst(\rH^i_\et(X_{y,\Kbar_v},\bQ_p)),\rF^\bullet\right) \cong \left(\sD_\pst(\rH^i_\et(X_{y_0,\Kbar_v},\bQ_p))),\Phi_{y_0}(y)\right)
\]
of filtered discrete $(\varphi,N,G_v)$-modules, where $\Phi_{y_0}\colon\Nbd_{y_0}\to\dG_{y_0}^\an$ is the period map associated to $\cH^i_\deR(X/Y)^\an$ (Definition~\ref{def:period_maps}) endowed with its Hodge filtration \todo{find citation that gives that graded pieces are vector bdles}.
\end{cor}

\alex{23/4}{We said we might try to rephrase this corollary in terms of a commuting square}

\subsubsection{Using period maps to prove finiteness}

For us, the significance of period maps is that they give us a mechanism for showing finiteness of subsets of~$Y(K_v)$ in the case that~$Y/K_v$ is a smooth projective curve.

\begin{lem}\label{lem:periods_prove_finiteness}
Suppose that~$Y/K_v$ is a smooth projective curve.
\begin{enumerate}[label=\roman*),ref=(\roman*)]
	\item\label{lempart:periods_prove_local_finiteness} Let $(V,\nabla,\rF^\bullet)$ be a filtered vector bundle with flat connection on~$Y^\an$, let~$y_0\in Y(K_v)$, and let $\Nbd_{y_0}\subseteq Y^\an$ be an admissible open neighbourhood of~$y_0$ isomorphic to a closed disc, over which $(V,\nabla)$ has a full basis of horizontal sections. Write
	\[
	\Phi_{y_0}\colon\Nbd_{y_0}\to\dG_{y_0}^\an
	\]
	for the period map associated to~$(V,\nabla,\rF^\bullet)$, and write~$\dZ_{y_0}\subseteq\dG_{y_0}$ for the Zariski-closure of the image of~$\Phi_{y_0}$, i.e.\ the smallest closed subvariety of~$\dG_{y_0}$ such that~$\Phi_{y_0}$ factors through~$\dZ_{y_0}^\an$.
	\smallskip

	Suppose that~$C_0\subseteq\Nbd_{y_0}(K_v)$ is a subset such that $\Phi_{y_0}(C_0)\subseteq\dG_{y_0}(K_v)$ is not Zariski-dense in~$\dZ_{y_0}$. Then~$C_0$ is finite.
	\item\label{lempart:compactness_gives_finiteness} Suppose that~$C\subseteq Y(K_v)$ is a subset such that every $y_0\in Y(K_v)$ has an admissible open neighbourhood~$\Nbd_{y_0}\subseteq Y^\an$ such that $C\cap\Nbd_{y_0}(K_v)$ is finite (e.g.\ using part~\ref{lempart:periods_prove_local_finiteness}). Then~$C$ is finite.
\end{enumerate}
\begin{proof}
\ref{lempart:periods_prove_local_finiteness} Choose a projective embedding $\dG_{y_0}\subseteq\bP^n_{K_v}$, and write the period map $\Phi_{y_0}$ in homogenous coordinates as $(\Phi_0:\Phi_1:\ldots:\Phi_n)$ with each~$\Phi_i$ a $K_v$-analytic function on~$\Nbd_{y_0}$. The fact that $\Phi_{y_0}(C_0)$ is not Zariski-dense in $\dZ_{y_0}$ implies that there is a homogenous polynomial $f\in K_v[X_0,\dots,X_n]$ which vanishes on $\Phi_{y_0}(C_0)$ but not on~$\dZ_{y_0}$. It follows that $f(\Phi_0,\dots,\Phi_n)$ is a non-zero analytic function on~$\Nbd_{y_0}$ which vanishes on~$C_0$. Since a non-zero $K_v$-analytic function on a closed disc has only finitely many zeroes~\cite[Theorem~2.2.9(1)]{fresnel-van_der_put:rigid_analytic_geometry}\footnote{In fact, \cite[Theorem~2.2.9(1)]{fresnel-van_der_put:rigid_analytic_geometry} shows that a non-zero $K_v$-analytic function on a closed disc has only finitely many zeroes over the completion of~$\Kbar_v$.}, it follows that~$C_0$ is finite.

\ref{lempart:compactness_gives_finiteness} This follows from the fact that each $\Nbd_{y_0}(K_v)$ is open in~$Y(K_v)$ for the $v$-adic topology \todo{?}, and that the latter is compact with respect to this topology. Note that the $K_v$-analytic subvarieties $\Nbd_{y_0}$ do not in general constitute an admissible covering of~$Y^\an$, even though their~$K_v$-points cover $Y(K_v)$.
\end{proof}
\end{lem}

%This lemma is the strategy employed by Lawrence and Venkatesh in their proof of the Mordell Conjecture \cite{LV}. To use Lemma~\ref{lem:periods_prove_finiteness} to prove finiteness of $Y(K)$ for $Y$ a smooth projective curve of genus~$\geq2$, one needs two ing

\subsection{Comparison with complex period maps}\label{ss:period_maps_complex}

In applying Lemma~\ref{lem:full_monodromy_gives_dense_image}, it will be important to be able to compute the Zariski-closure of the image of the period map
\[
\Phi_{y_0}\colon\Nbd_{y_0}\to\dG_{y_0}^\an
\]
associated to an \emph{algebraic} filtered vector bundle with flat connection $(V,\nabla,\rF^\bullet)$ on a smooth $K_v$-variety~$Y$.% For simplicity, we discuss here only the case when $(V,\nabla,\rF^\bullet)$ is the relative de Rham cohomology of a smooth proper family $X\to Y$ with its Gau\ss--Manin connection and Hodge filtration, though a similar discussion holds in general.

The way one typically controls the image of the period map is via comparing with a complex-analytic version of the period map, which can be controlled via monodromy computations. The complex-analytic period map is defined as follows.

\begin{defi}\label{def:period_map_complex}
Let~$Y$ be a smooth variety over~$\bC$ with a point $y_0\in Y(\bC)$, and write~$Y^\an$ for the complex analytification of~$Y$. Let $\Nbd_{y_0}\to Y^\an$ be a local biholomorphism of complex manifolds with $\Nbd_{y_0}$ simply connected (e.g.\ the inclusion of a polydisc neighbourhood of~$y_0$, or the universal cover of a component of~$Y^\an$), and let~$\tilde y_0\in\Nbd_{y_0}$ be a preimage of~$y_0$.

Then for any holomorphic vector bundle $(V,\nabla)$ on~$Y^\an$, the pullback $(V|_{\Nbd_{y_0}},\nabla|_{\Nbd_{y_0}})$ to~$\Nbd_{y_0}$ is a vector bundle with flat connection on a simply connected complex manifold, and hence by the Riemann--Hilbert correspondence there is a unique isomorphism
\[
T_{\tilde y_0}^\nabla\colon(\cO_{\Nbd_{y_0}}\otimes_\bC V_{y_0},\rd\otimes1)\xrightarrow\sim(V|_{\Nbd_{y_0}},\nabla|_{\Nbd_{y_0}})
\]
of vector bundles with flat connection on $\Nbd_{y_0}$, characterised by the fact that its fibre at $\tilde y_0$ is the identity.

Suppose moreover that~$V$ carries an exhaustive, separated filtration $\dots\geq\rF^1V\geq\rF^0V\geq\rF^{-1}V\geq\dots$ (not necessarily stable under the connection~$\nabla$) whose graded pieces are all vector bundles. We define the \emph{period domain} $\dG_{y_0}$ to be the complex flag variety parametrising filtrations on $V_{y_0}$ with the same dimension data as $\rF^\bullet V_{y_0}$, and define the (complex) \emph{period map} to be the holomorphic map
\[
\Phi_{\tilde y_0}\colon\Nbd_{y_0}\to\dG_{y_0}^\an
\]
classifying the filtration on $\cO_{\Nbd_{y_0}}\otimes_\bC V_{y_0}$ given by pulling back the filtration~$\rF^\bullet$ along the parallel transport map~$T_{\tilde y_0}^\nabla$.
\end{defi}

\todo{find reference for complex version of \cite{conrad:analytification}?}

Although $v$-adic and complex period maps appear to be very different kinds of objects, there is in fact a comparison isomorphism relating them.

\begin{thm}[Comparison for period maps]\label{thm:period_comparison}
Let~$Y$ be a smooth $K_v$-variety, and let $(V,\nabla,\rF^\bullet)$ be a filtered (algebraic) vector bundle with flat connection on~$Y$ (e.g.\ the relative de Rham cohomology of a smooth proper morphism $\pi\colon X\to Y$). Let $y_0\in Y(K_v)$, and fix an embedding $\iota\colon K_v\hookrightarrow\bC$. Fix:
\begin{itemize}
	\item an admissible open neighbourhood $\Nbd_{y_0,v}\subseteq Y^\an$ in the rigid analytification~$Y^\an$ of~$Y$, isomorphic to a closed polydisc, over which $(V,\nabla)^\an$ has a full basis of horizontal sections; and
	\item a local biholomorphism $\Nbd_{y_0,\infty}\to Y_\bC^\an$ to the complex analytification~$Y_\bC^\an$ of~$Y_\bC$ with $\Nbd_{y_0,\infty}$ simply connected, along with a point $\tilde y_0$ in the preimage of~$y_0$.
\end{itemize}

Let~$\dG_{y_0}$ denote the flag variety over $K_v$ parametrising filtrations on $V_{y_0}$ with the same dimension data as $\rF^\bullet V_{y_0}$. Let~$\dZ_{y_0,v}\subseteq\dG_{y_0}$ denote the Zariski-closure of the image of the $v$-adic period map $\Phi_{y_0,v}\colon\Nbd_{y_0,v}\to\dG_{y_0}^\an$, and let~$\dZ_{y_0,\infty}\subseteq\dG_{y_0,\bC}$ denote the Zariski-closure of the image of the complex-analytic period map $\Phi_{\tilde y_0,\infty}\colon\Nbd_{y_0,\infty}\to\dG_{y_0,\bC}^\an$. Then~$\dZ_{y_0,\infty}$ is the base-change of~$\dZ_{y_0,v}$ from~$K_v$ to~$\bC$ along~$\iota$.
\end{thm}

\begin{proof}
This is essentially proved in \cite[\S3.4]{LV}, except that there the variety~$Y$ and point~$y_0$ are defined over the number field~$K$. For the sake of completeness, we give the argument here, which is a straightforward modification of that in \cite{LV}.

\smallskip

Firstly, we note that the subvariety $\dZ_{y_0,v}\subseteq\dG_{y_0}$ doesn't depend on the particular choice of neighbourhood~$\Nbd_{y_0,v}$. Indeed, suppose that $\Nbd_{y_0,v}'\subseteq\Nbd_{y_0,v}$ is a smaller admissible polydisc neighbourhood of~$y_0$, and write $\Phi_{y_0,v}'\colon\Nbd_{y_0,v}'\to\dG_{y_0}^\an$ for the $v$-adic period map on $\Nbd_{y_0,v}'$ and $\dZ_{y_0,v}'$ for the Zariski-closure of its image. It follows from the construction that $\Phi_{y_0,v}'$ is just the restriction to~$\Nbd_{y_0,v}$ of the period map $\Phi_{y_0,v}$, from which it follows that $\dZ_{y_0,v}'\subseteq\dZ_{y_0,v}$. For the converse inclusion, we observe as in the proof of Lemma~\ref{lem:periods_prove_finiteness} that $\Phi_{y_0,v}^{-1}(\dZ_v'^\an)$ is the vanishing locus of a set of $K_v$-analytic functions on the disc $\Nbd_{y_0,v}$ and contains the open subdisc $\Nbd_{y_0,v}'$. It follows from the identity principle that $\Phi_{y_0,v}^{-1}(\dZ_v'^\an)=\Nbd_{y_0,v}$, whence $\dZ_{y_0,v}\subseteq\dZ_{y_0,v}'$.

Now by a similar argument, we see that the Zariski-closure of the image of the complex period map $\Phi_{\tilde y_0,\infty}\colon\Nbd_{y_0,\infty}\to\dG_{y_0,\bC}^\an$ doesn't depend on the choice of $\Nbd_{y_0,\infty}$. Hence, shrinking $\Nbd_{y_0,v}$, $\Nbd_{y_0,\infty}$ and~$Y$ if necessary, it suffices to prove Theorem~\ref{thm:period_comparison} in the special case that $V=\cO_Y^{\oplus m}$ is the constant (algebraic) vector bundle of some rank~$m$, and that each $\rF^iV=\cO_Y^{\oplus m_i}$ is the constant subbundle spanned by the first~$m_i$ basis sections, where~$m_i=\rank\rF^iV$. We also fix a system $t_1,\dots,t_d$ of (algebraic) local parameters at~$y_0$, and assume without loss of generality that $\Nbd_{y_0,v}=\Sp(K_v\langle t_1,\dots,t_d\rangle)$ is the closed rigid polydisc of radii $1$ in the local parameters $t_1,\dots,t_d$, and that $\Nbd_{y_0,\infty}\to Y_\bC$ is an open immersion of the open complex polydisc of radii $1$ in the local parameters $t_1,\dots,t_d$ (so~$y_0$ has a unique preimage~$\tilde y_0=y_0$).

Now the connection $\nabla$ on~$V=\cO_Y^{\oplus m}$ is given by $\nabla(\underline f)=\rd(\underline f)+\uunderline\omega\cdot\underline f$, where the connection matrix $\uunderline\omega$ is an $m\times m$ matrix with coefficients in $\Gamma(Y,\Omega^1_{Y/K_v})$. (Flatness of the connection is equivalent to the equality $\rd\uunderline\omega+\uunderline\omega\wedge\uunderline\omega=0$.) \cite[Proposition~8.9]{katz:nilpotent_connections} ensures that there is a \emph{unique} $m\times m$ matrix $\uunderline T$ with coefficients in $K_v\llbrack t_1,\dots,t_d\rrbrack$ satisfying the differential equation
\begin{equation}\label{eq:de_for_parallel_transport}
\rd\uunderline T=-\uunderline\omega\cdot\uunderline T\;\text{ subject to the initial condition }\;\uunderline T|_{t_1=\dots=t_d=0} = \mathbf I_m \,,
\end{equation}
where $\rd\colon K_v\llbrack t_1,\dots,t_d\rrbrack\to\Omega^f_{K_v\llbrack t_1,\dots,t_d\rrbrack/K_v}=\bigoplus_{i=1}^dK_v\llbrack t_1,\dots,t_d\rrbrack\rd t_i$ is the universal continuous/finite\todo{decide} derivation. Here, by mild abuse of notation, we regard $\uunderline\omega$ as a matrix with coefficients in $\Omega^f_{K_v\llbrack t_1,\dots,t_d\rrbrack/K_v}$ via the inclusion $\Gamma(Y,\Omega^1_{Y/K_v})\hookrightarrow\Omega^f_{K_v\llbrack t_1,\dots,t_d\rrbrack/K_v}$.

For $1\leq i\leq m$ we write $\underline T_i$ for the $i$th column of $\uunderline T$, and let
\[
\Phi_{y_0,\infsml}\colon\Spec(K_v\llbrack t_1,\dots,t_d\rrbrack)\to\dG_{y_0}
\]
denote the $K_v$-scheme map classifying the filtration on $K_v\llbrack t_1,\dots,t_d\rrbrack^{\oplus m}$ where $\rF^i$ is the span of the vectors $\underline T_1,\dots,\underline T_{m_i}$. Explicitly, the flag variety $\dG_{y_0}$ is a closed subvariety of $\prod_{i\in\bZ}\bP_{K_v}^{{m\choose m_i}-1}$ via the embedding taking a filtration~$\rF^\bullet$ on $K_v^{\oplus m}$ to the sequence of one-dimensional subspaces $\bigwedge^{m_i}\rF^i\leq\bigwedge^{m_i}(K_v^{\oplus m})=K_v^{\oplus{m\choose m_i}}$, and $\Phi_{y_0,\infsml}$ is the map whose $i$th component is given by $\underline T_1\wedge\dots\wedge\underline T_{m_i}$, viewed as a map from $K_v\llbrack t_1,\dots,t_d\rrbrack\to\bA^{m\choose m_i}\setminus\{0\}$.

\smallskip

Now the sheaf of $K_v$-analytic $1$-forms on~$\Nbd_{y_0,v}$ is the free vector bundle generated by $\rd t_1,\dots,\rd t_d$ \cite[Proof of Theorem~3.6.1]{fresnel-van_der_put:rigid_analytic_geometry}, so the $v$-adic parallel transport map
\[
T_{y_0,v}^\nabla\colon(\cO_{\Nbd_{y_0,v}}^{\oplus m},\rd^{\oplus m})\xrightarrow\sim(\cO_{\Nbd_{y_0,v}}^{\oplus m},\nabla)
\]
is represented by an $m\times m$ matrix with coefficients in $K_v\langle t_1,\dots,t_d\rangle\subset K_v\llbrack t_1,\dots,t_d\rrbrack$ which satisfies the differential equation~\eqref{eq:de_for_parallel_transport}. It thus follows by unicity of solutions to~\eqref{eq:de_for_parallel_transport} that $T_{y_0,v}^\nabla$ is represented by the matrix~$\uunderline T$ (which thus has coefficients in $K_v\langle t_1,\dots,t_d\rangle$). It then follows that the $v$-adic period map
\[
\Phi_{y_0,v}\colon\Nbd_{y_0,v}\to\dG_{y_0}^\an\subseteq\prod_{i\in\bZ}\bP_{K_v}^{{m\choose m_i}-1,\an}
\]
is the map whose $i$th component is given by $\underline T_1\wedge\dots\wedge\underline T_{m_i}$: in other words, the Taylor expansion of $\Phi_{y_0,v}$ at $y_0$ is the map $\Phi_{y_0,\infsml}$. Using this, we see

\begin{prop}\label{prop:v-adic_image_is_formal}
The Zariski-closure~$\dZ_{y_0,v}$ of the image of the $v$-adic period map $\Phi_{y_0,v}\colon\Nbd_{y_0,v}\to\dG_{y_0}^\an$ is the scheme-theoretic image of the formal period map $\Phi_{y_0,\infsml}$.
\begin{proof}
Choose a projective embedding $\dG_{y_0}\subseteq\bP_{K_v}^N$. The above discussion shows that there are elements $f_0,\dots,f_N\in K_v\langle t_1,\dots,t_d\rangle$ such that both the $v$-adic period map $\Phi_{y_0,v}\colon\Nbd_{y_0,v}\to\dG_{y_0}^\an$ and the formal period map $\Phi_{y_0,\infsml}\colon\Spec(K_v\llbrack t_1,\dots,t_d\rrbrack)\to\dG_{y_0}$ are given in projective coordinates by $(f_0:\ldots:f_N)$. The homogenous ideal of definition of~$\dZ_{y_0,v}\subseteq\bP^N_{K_v}$ is then the ideal generated by those homogenous elements $F\in K_v[X_0,\dots,X_N]$ such that $F(f_0,\dots,f_N)=0$. But this is also the homogenous ideal of definition of the scheme-theoretic image of~$\Phi_{y_0,\infsml}$.
\end{proof}
\end{prop}

We can apply exactly the same argument to the complex-analytic period map. The embedding $\iota\colon K_v\hookrightarrow\bC$ induces an embedding $K_v\llbrack t_1,\dots,t_d\rrbrack\hookrightarrow\bC\llbrack t_1,\dots,t_d\rrbrack$, which we also denote by~$\iota$. The sheaf of holomorphic $1$-forms on the polydisc $\Nbd_{y_0,\infty}$ is the free vector bundle generated by $\rd t_1,\dots,\rd t_d$, whence the complex-analytic parallel transport map
\[
T_{y_0,\infty}^\nabla\colon(\cO_{\Nbd_{y_0,\infty}}^{\oplus m},\rd^{\oplus m})\xrightarrow\sim(\cO_{\Nbd_{y_0,\infty}}^{\oplus m},\nabla)
\]
is represented by an $m\times m$ matrix $\uunderline T_\infty$ with coefficients in the ring $\cO(\Nbd_{y_0,\infty})\subset\bC\llbrack t_1,\dots,t_d\rrbrack$ of holomorphic functions on the polydisc of radii~$1$ which satisfies the differential equation
\[
\rd\uunderline T_\infty=-\iota(\uunderline\omega)\cdot\uunderline T_\infty\;\text{ subject to the initial condition }\;\uunderline T_\infty|_{t_1=\dots=t_d=0} = \mathbf I_m \,.
\]
Since this differential equation has a unique solution over $\bC\llbrack t_1,\dots,t_d\rrbrack$, it follows that $\uunderline T_\infty=\iota(\uunderline T)$. It then follows that the complex-analytic period map
\[
\Phi_{y_0,\infty}\colon\Nbd_{y_0,\infty}\to\dG_{y_0,\bC}^\an\subseteq\prod_{i\in\bZ}\bP_\bC^{{m\choose m_i}-1,\an}
\]
is the map whose $i$th component is given by $\iota(\underline T_1)\wedge\dots\wedge\iota(\underline T_{m_i})$. As for the~$v$-adic period map, this implies

\begin{prop}\label{prop:complex_image_is_formal}
The Zariski-closure~$\dZ_{y_0,\infty}$ of the image of the complex-analytic period map $\Phi_{y_0,\infty}\colon\Nbd_{y_0,\infty}\to\dG_{y_0,\bC}^\an$ is the scheme-theoretic image of the formal period map $\Phi_{y_0,\infsml}\circ\iota\colon\Spec(\bC\llbrack t_1,\dots,t_d\rrbrack)\to\dG_{y_0,\bC}$.
\begin{proof}
The same proof as Proposition~\ref{prop:v-adic_image_is_formal} works with only minor modifications.
\end{proof}
\end{prop}

Combining Proposition~\ref{prop:v-adic_image_is_formal} and~\ref{prop:complex_image_is_formal} then yields Theorem~\ref{thm:period_comparison}. Consider the commuting square
\begin{center}
\begin{tikzcd}
\Spec(\bC\llbrack t_1,\dots,t_d\rrbrack) \arrow[r,"\Phi_{y_0,\inf}\circ\iota"]\arrow[d,"\iota"] & \dG_{y_0,\bC} \arrow[d] \\
\Spec(K_v\llbrack t_1,\dots,t_d\rrbrack) \arrow[r,"\Phi_{y_0,\infsml}"] & \dG_{y_0}
\end{tikzcd}
\end{center}
of $K_v$-schemes, in which the scheme-theoretic image of the bottom and top maps are~$\dZ_{y_0,v}$ and~$\dZ_{y_0,\infty}$, respectively. It follows that the top arrow factors as
\[
\Spec(\bC\llbrack t_1,\dots,t_d\rrbrack)\to\Spec(\bC\otimes_{K_v}K_v\llbrack t_1,\dots,t_d\rrbrack)\xrightarrow{\bC\otimes\Phi_{y_0,\infsml}}\dZ_{y_0,v,\bC}\hookrightarrow\dG_{y_0,\bC} \,.
\]
The first and second of these maps are scheme-theoretically dense\footnote{A morphism $f\colon U\to V$ of schemes is \emph{scheme-theoretically dense} just when the map $\cO_V\hookrightarrow f_*\cO_U$ is injective. In our particular case, all schemes appearing are reduced, so this is equivalent to the maps in question being dominant.} (using that $\iota\colon K_v\hookrightarrow\bC$ is flat for the second). It follows that $\Phi_{y_0,\infsml,\bC}\colon\Spec(\bC\llbrack t_1,\dots,t_d\rrbrack)\to\dZ_{y_0,v,\bC}$ is scheme-theoretically dense, so that $\dZ_{y_0,\infty}=\dZ_{y_0,v,\bC}$ as claimed.
\end{proof}

\begin{rmk}
When the smooth variety~$Y$, the point~$y_0$ and the filtered vector bundle with flat connection~$(V,\nabla,\rF^\bullet)$ are all defined over the number field~$K$, then the formal period map $\Phi_{y_0,\infsml}$ is also defined over~$K$. More precisely, if we choose the trivialisation of~$(V,\rF^\bullet)$ to be defined over~$K$, then the coefficients of the matrix $\uunderline T$ lie in $K\llbrack t_1,\dots,t_d\rrbrack$.
\end{rmk}

\subsubsection{Monodromy}

Over the complex numbers, period maps can be controlled by monodromy computations. For the sake of simplicity, we restrict here to discussing the case of relative de Rham cohomology, though a similar discussion is valid in general. Suppose that $f\colon X\to Y$ is a smooth proper morphism of $\bC$-varieties, and let~$y_0\in Y^\an$ be a fixed basepoint. The derived pushforward $\rR^if^\an_*\ubQ_{X^\an}$ of the constant sheaf~$\ubQ_{X^\an}$ on~$X^\an$ is a $\bQ$-local system\footnote{The fact that the pushforward is a local system follows from Ehresmann's Theorem that $f^\an$ is a locally trivial fibration \cite{ehresmann:fibrations}, plus the proper base change theorem from topology \cite[Theorem~17.3]{milne:etale}.} on~$Y^\an$ whose fibre over~$y_0$ is the derived functor\footnote{The derived functor cohomology is canonically isomorphic to the usual singular/Betti cohomology $\rH^i_\sing(X_{y_0}^\an,\bQ)$ of~$X_{y_0}^\an$. The authors don't know of a good reference for this fact, but it is a straightforward consequence of the fact that the complex $\cC^\bullet_{X^\an}(-,\bQ)$ of sheaves of singular cochains on~$X^\an$ is a resolution of the constant sheaf~$\ubQ_{X^\an}$ by flabby sheaves.} cohomology~$\rH^i(X_{y_0}^\an,\bQ)$ of the fibre~$X_{y_0}^\an$ \cite[Theorem~17.2]{milne:etale}. It follows that there is a $\bQ$-linear monodromy action of the fundamental group $\pi_1(Y^\an,y_0)$ on $\rH^i(X_{y_0}^\an,\bQ)$. This induces a monodromy action on the set of $\bC$-linear filtrations on $\bC\otimes_\bQ\rH^i(X_{y_0}^\an,\bQ)\cong\rH^i_\deR(X_{y_0}/\bC)$, and hence on the period domain $\dG_{y_0}$ classifying filtrations on $\rH^i_\deR(X_{y_0}/\bC)$ with the same dimension data as the Hodge filtration. This action is related to the complex-analytic period map as follows.

\begin{lem}\label{lem:monodromy_bounds_complex_period_map}
Suppose that $\Nbd_{y_0}\to Y^\an$ is a local biholomorphism of complex manifolds with $\Nbd_{y_0}$ simply connected, and let $\tilde y_0\in\Nbd_{y_0}$ be a preimage of~$y_0$. Then the Zariski-closure of the image of the complex-analytic period map
\[
\Phi_{y_0}\colon\Nbd_{y_0}\to\dG_{y_0}^\an
\]
from Definition~\ref{def:period_map_complex} contains the $\pi_1(Y^\an,y_0)$-orbit of the point $h_0\in\dG_{y_0}(\bC)$ corresponding to the Hodge filtration on $\rH^i_\deR(X_{y_0}/\bC)$.
\end{lem}

Combined with Theorem~\ref{thm:period_comparison}, this yields

\begin{cor}[Controlling the $v$-adic period map via monodromy {\cite[Lemma~3.3]{LV}}]
Let~$X\to Y$ be a proper smooth morphism of smooth $K_v$-varieties, and let~$y_0\in Y(K_v)$. Choose an admissible open neighbourhood $\Nbd_{y_0}\subseteq Y^\an$ in the rigid analytification~$Y^\an$ of~$Y$, isomorphic to a closed polydisc, over which $\cH^i_\deR(X/Y)^\an$ has a full basis of horizontal sections, and a complex embedding $\iota\colon K_v\hookrightarrow\bC$.

Then the $K_v$-dimension of the Zariski-closure of the image of the $v$-adic period map $\Phi_{y_0}\colon\Nbd_{y_0}\to\dG_{y_0}^\an$ is greater than or equal to the $\bC$-dimension of the Zariski-closure of the $\pi_1(Y_\bC^\an,y_0)$-orbit of the point $h_0\in\dG_{y_0,\bC}$ corresponding to the Hodge filtration on~$\rH^i_\deR(X_{y_0,\bC}/\bC)$.
\end{cor}

To prove Lemma~\ref{lem:monodromy_bounds_complex_period_map}, we note that the holomorphic vector bundle with connection $\cH^i_\deR(X/Y)^\an$ and the $\bC$-local system $\rR^if^\an_*\ubC_{X^\an}$ correspond to one another under the Riemann--Hilbert correspondence: explicitly, there is an isomorphism $\rR^if^\an_*\ubC_{X^\an}\cong\cH^i_\deR(X/Y)^{\an,\nabla=0}$ whose fibre at~$y_0$ recovers the comparison isomorphism $\rH^i(X_{y_0}^\an,\bC)\cong\rH^i_\deR(X_{y_0}/\bC)$. This isomorphism arises from the morphisms
\begin{equation}\label{eq:relative_cohomology_comparison_complex}\tag{$\dag$}
\rR^i f^\an_*\ubC_{X^\an} \rightarrow \cH^i_\deR(X^\an/Y^\an) \leftarrow \cH^i_\deR(X/Y)^\an \,,
\end{equation}
where the left-hand arrow is induced from the map $\ubC_{X^\an}\to\Omega_{X^\an/Y^\an}^\bullet$ of the constant sheaf into the complex of sheaves of relative differential forms, and the right-hand arrow is the base-change map\todo{I think I'm implicitly using some coherence result for base-change maps} from the commuting square
\begin{center}
\begin{tikzcd}
X^\an \arrow[d,"f^\an"]\arrow[r] & X \arrow[d,"f"] \\
Y^\an \arrow[r] & Y
\end{tikzcd}
\end{center}
of locally-ringed spaces, applied to the complex $\Omega_{Y/X}^\bullet$. Since the map $\ubC_{X^\an}\to\Omega_{X^\an/Y^\an}^\bullet$ factors through $\Omega_{X^\an/\bC}^\bullet$, the image of the left-hand map is contained in the kernel of the Gau\ss--Manin connection~$\nabla$.

Taking the fibre of~\eqref{eq:relative_cohomology_comparison_complex} at a point $y\in Y^\an$ yields the usual comparison isomorphisms
\[
\rH^i(X_y^\an,\bC) \xrightarrow\sim \rH^i_\deR(X_y^\an/\bC) \xleftarrow\sim \rH^i_\deR(X_y/\bC)
\]
between derived functor cohomology, analytic de Rham cohomology and algebraic de Rham cohomology \cite[Theorem~1']{grothendieck:de_rham_cohomology}. Since the maps in~\eqref{eq:relative_cohomology_comparison_complex} are fibrewise isomorphisms, it follows that the right-hand map is an isomorphism of holomorphic vector bundles with flat connection, and the left-hand map induces an isomorphism of $\bC$-local systems from $\rR^if^\an_*\ubC_{X^\an}$ to the local system of horizontal sections of $\cH^i_\deR(X^\an/Y^\an)$. Thus composing the two maps in~\eqref{eq:relative_cohomology_comparison_complex} yields the claimed isomorphism $\rR^if^\an_*\ubC_{X^\an}\cong\cH^i_\deR(X/Y)^{\an,\nabla=0}$.

\smallskip

Now we saw in the proof of Theorem~\ref{thm:period_comparison} that the Zariski-closure of the image of the complex period map $\Phi_{\tilde y_0}$ doesn't depend on the choice of local biholomorphism $\Nbd_{y_0}\to Y^\an$, and hence in proving Lemma~\ref{lem:monodromy_bounds_complex_period_map} we may assume that $\Nbd_{y_0}\to Y^\an$ is a universal cover of the connected component containing~$y_0$ (endowed with the point~$\tilde y_0$ over~$y_0$). If $\gamma\in\pi_1(Y^\an,y_0)$ is an element of the fundamental group, then we may lift $\gamma$ uniquely to a path in~$\Nbd_{y_0}$

Path-lifting then provides a set-map $\pi_1(Y^\an,y_0)\to\Nbd_{y_0}$, identifying $\pi_1(Y^\an,y_0)$ with the fibre of~$\Nbd_{y_0}$ over~$y_0$. If $\gamma\in\pi_1(Y^\an,y_0)$ corresponds to the point~$\tilde y_0'\in\Nbd_{y_0}$ lying over~$y_0$, then it follows from the isomorphism $\rR^if^\an_*\ubC_{X^\an}\cong\cH^i_\deR(X/Y)^\an$ that the monodromy action of $\gamma$ on $\rH^i(X_{y_0}^\an,\bC)\cong\rH^i_\deR(X_{y_0}/\bC)^\an$ is given by the parallel transport map $T_{\tilde y_0,\tilde y_0'}^\nabla\colon\rH^i_\deR(X_{y_0}/\bC)\xrightarrow\sim\rH^i_\deR(X_{y_0}/\bC)$ (fibre of $T_{\tilde y_0}^\nabla$ from \todo{ref} at~$\tilde y_0'$). In the language of period maps, this says that
\[
\Phi_{\tilde y_0}(\tilde y_0') = \gamma^{-1}h_0\,.
\]
Thus, we see that the $\pi_1(Y^\an,y_0)$-orbit~$h_0$ is contained in the image of the period map, and we have proved Lemma~\ref{lem:monodromy_bounds_complex_period_map}.

\subsection{Local systems and lisse sheaves}\label{ss:local_systems}

\alex{02/09}{Write this section. Include universal covers, and that they determine fibre functors. Also allow fibre functors defined over rings where all finite \'etale extensions are split?}

\begin{lem}\label{lem:analytic_and_algebraic_pi_1}
Let~$A$ be a strictly affinoid $K_v$-algebra, with associated affinoid $K_v$-analytic space~$\Sp(A)$. Then the functor $B\mapsto\Sp(B)$ provides a contravariant equivalence of categories between finite \'etale $A$-algebras and finite \'etale coverings of~$\Sp(A)$.

In particular, if~$A$ is an integral domain and $\bar\eta\colon A\to\Omega$ is a $K_v$-algebra homomorphism from~$A$ into a complete algebraically closed field, then there is a canonical isomorphism
\[
\pi_1^\alg(\Sp(A),\bar\eta) \cong \pi_1^\et(\Spec(A),\bar\eta) \,.
\]
\begin{proof}
\cite[Definition~4.5.7]{fresnel-van_der_put:rigid_analytic_geometry} and the result just below it show that $B\mapsto\Sp(B)$ gives an equivalence between finite $A$-algebras and $K_v$-analytic spaces finite over~$\Sp(A)$. Part~(1) of the proof of \cite[Proposition~8.1.1]{fresnel-van_der_put:rigid_analytic_geometry} shows that a morphism $\Sp(B)\to\Sp(A)$ of affinoid $K_v$-analytic spaces is \'etale if and only if~$B$ is a flat $A$-algebra and the module $\Omega_{B/A}^f$ of finite differentials is zero. In the particular case that~$B$ is a finite $A$-algebra, the module~$\Omega_{B/A}^1$ of K\"ahler differentials is finite, whence $\Omega_{B/A}^f=\Omega_{B/A}^1$. We conclude that a finite morphism $\Sp(B)\to\Sp(A)$ is \'etale just when~$B$ is flat over~$A$ and $\Omega^1_{B/A}=0$; that is to say, just when~$B$ is an \'etale $A$-algebra.
\end{proof}
\end{lem}

\subsection{Some relative $p$-adic Hodge theory}\label{ss:relative_p-adic_hodge}

We conclude this section with the proof of Theorem~\ref{thm:period_maps_control_reps}. As we mentioned before, when $X\to Y$ has suitably good reduction at~$v$, this can be proved by relating both \'etale and de Rham cohomology to the crystalline cohomology of the special fibre of~$X_{y_0}$. However, in the absence of any assumptions on the reduction type of $X\to Y$, we are forced to take a different approach, using the relative $p$-adic Hodge theory of Scholze \cite{scholze:relative_p-adic_hodge_theory}.

We recall some of the basics. Let~$U$ be a smooth $K_v$-analytic space. Scholze associates to~$U$ a site~$U_\proet$, called the pro-\'etale site \cite[Definition~3.9]{scholze:relative_p-adic_hodge_theory}\cite[Erratum~(1)]{scholze:relative_p-adic_hodge_theory_erratum}. This site carries several important sheaves of $\bZ_p$-algebras, including:
\begin{itemize}
	\item the structure sheaf~$\cO_U$ (a sheaf of $K_v$-algebras);
	\item the sheaf~$\hat\bZ_{p,U}:=\varprojlim(\underline{\bZ/p^n}_U)$ where $\underline{\bZ/p^n}_U$ denotes the constant sheaf on~$U$ ($\hat\bZ_{p,U}$ is not the constant sheaf with value~$\bZ_p$, but plays a very similar role) \cite[Definition~8.1]{scholze:relative_p-adic_hodge_theory};
	\item the \emph{positive de Rham sheaf} $\bB_{\deR,U}^+$ \cite[Definition~6.1(ii)]{scholze:relative_p-adic_hodge_theory}, which is a sheaf of $\hat\bZ_{p,U}$-algebras; and
	\item the \emph{structural de Rham sheaf} $\cO\bB_{\deR,U}$ \cite[Definition~6.8(iv)]{scholze:relative_p-adic_hodge_theory}\cite[Erratum~(3)]{scholze:relative_p-adic_hodge_theory_erratum}, which is a sheaf of filtered $\cO_U$-algebras endowed with a flat connection
	\[
	\nabla\colon\cO\bB_{\deR,U}\to\Omega^1_{U/K_v}\otimes_{\cO_U}\cO\bB_{\deR,U}
	\]
	satisfying the Leibniz rule $\nabla(fg)=\nabla(f)g+\nabla(g)f$, extending the connection~$\rd$ on~$\cO_U$, and satisfying Griffiths transversality with respect to the filtration~$\rF^\bullet$. The positive de Rham period sheaf~$\bB_{\deR,U}^+=(\rF^0\!\cO\bB_{\deR,U})^{\nabla=0}$ is the sheaf of horizontal sections of~$\rF^0\!\cO\bB_{\deR,U}$ \cite[Proof of Lemma~7.7]{scholze:relative_p-adic_hodge_theory}.
\end{itemize}

These sheaves of algebras allow one to identify several important categories of sheaves on $U_\proet$.

\begin{defi}[Local systems and vector bundles]
\leavevmode
\begin{enumerate}
	\item A \emph{$\hat\bZ_p$-local system} on~$U$ is a sheaf~$\bL$ of~$\hat\bZ_{p,U}$-modules which, locally on~$U_\proet$, is isomorphic to the sheaf $\hat\bZ_{p,U}\otimes_{\bZ_p}M$ for a finitely generated $\bZ_p$-module~$M$ \cite[Definition~8.1]{scholze:relative_p-adic_hodge_theory}.
	\item A \emph{$\bB_\deR^+$-local system} on~$U$ is a sheaf~$\bM$ of~$\bB_{\deR,U}^+$-modules which, locally on~$U_\proet$, is free of finite rank \cite[Definition~7.1]{scholze:relative_p-adic_hodge_theory}.
	\item A \emph{filtered vector bundle with flat connection} on~$U$ is a locally finite free sheaf~$\dE$ of $\cO_U$-modules, together with an exhaustive, separated decreasing filtration $\rF^\bullet\!\dE$ whose graded pieces are all locally free $\cO_U$-modules, and a flat connection
	\[
	\nabla\colon\dE\to\Omega^1_{U/K_v}\otimes_{\cO_U}\dE
	\]
	satisfying the Leibniz rule with respect to the connection~$\rd$ on~$\cO_U$ and Griffiths transversality with respect to the filtration~$\rF^\bullet$ \cite[Definition~7.4]{scholze:relative_p-adic_hodge_theory}.
	\item A \emph{filtered $\cO\bB_\deR$-module with flat connection} on~$U$ is a sheaf~$\dM$ of filtered~$\cO\bB_{\deR,U}$-modules which, locally on~$U_\proet$, is filtered-isomorphic to $\cO\bB_{\deR,U}^{\oplus m}$ for some~$m$, together with a flat connection
	\[
	\nabla\colon\dM\to\Omega^1_{U/K_v}\otimes_{\cO_U}\dM
	\]
	satisfying the Leibniz rule with respect to the connection~$\nabla$ on~$\cO\bB_{\deR,U}$ and Griffiths transversality with respect to the filtration~$\rF^\bullet$ on~$\dM$.
\end{enumerate}
\end{defi}

%\begin{rmk}
%The category~$\Loc_{\hat\bZ_p}(U)$ is $\otimes$-equivalent to the category of~$\bZ_p$-local systems on~$U_\et$ \cite[Proposition~8.2]{scholze:relative_p-adic_hodge_theory}.
%\end{rmk}

We write~$\Loc_{\hat\bZ_p}(U)$, $\Loc_{\bB_\deR^+}(U)$, $\FMIC(U)$ and $\FMIC_{\cO\bB_\deR}(U)$ for the $\otimes$-categories of $\hat\bZ_p$-local systems, $\bB_\deR^+$-local systems, filtered vector bundles with flat connection, and filtered $\cO\bB_\deR$-modules with flat connection on~$U$, respectively. There are $\bZ_p$-linear $\otimes$-functors
\begin{equation}\label{eq:base-change_functors}
\Loc_{\hat\bZ_p}(U) \rightarrow \Loc_{\bB_\deR^+}(U) \rightarrow \FMIC_{\cO\bB_\deR}(U) \leftarrow \FMIC(U)
\end{equation}
given by base change along the morphisms\footnote{There is a small thing to be checked here: that if $\dE$ is a filtered vector bundle with flat connection on~$U$, then $\cO\bB_{\deR,U}\otimes_{\cO_U}\dE$ is locally filtered-isomorphic to~$\cO\bB_{\deR,U}^{\oplus m}$ for some~$m$. This follows from the fact that~$\dE$ and all graded pieces of its filtration are locally free of finite rank, and the fact that, locally on~$U_\proet$, there is a section~$t$ of~$\cO\bB_{\deR,U}$ such that multiplication by~$t$ gives a filtered isomorphism~$\cO\bB_{\deR,U}\xrightarrow\sim\cO\bB_{\deR,U}$ of degree~$1$.}
\[
\hat\bZ_{p,U} \hookrightarrow \bB_{\deR,U}^+ \hookrightarrow \cO\bB_{\deR,U} \hookleftarrow \cO_U \,.
\]

\begin{prop}\label{prop:p-adic_riemann-hilbert}
The functors $\Loc_{\bB_\deR^+}(U) \hookrightarrow \FMIC_{\cO\bB_\deR}(U) \hookleftarrow \FMIC(U)$ are fully faithful, and the image of $\FMIC(U)\hookrightarrow\FMIC_{\cO\bB_\deR}(U)$ is contained in the essential image of $\Loc_{\bB_\deR^+}(U) \hookrightarrow \FMIC_{\cO\bB_\deR}(U)$.
\begin{proof}
Let $\dI\subseteq\FMIC_{\cO\bB_\deR}(U)$ denote the full subcategory consisting of those filtered $\cO\bB_\deR$-modules with flat connection~$\dM$ such that\footnote{The authors do not know whether this condition is in fact true for all~$\dM\in\FMIC_{\cO\bB_\deR}(U)$.}~$\rF^0\!\dM^{\nabla=0}$ is a $\bB_\deR^+$-local system on~$U$ (for the natural~$\bB_{\deR,U}^+=\rF^0\!\cO\bB_{\deR,U}^{\nabla=0}$-module structure). The proof of \cite[Theorem~7.6(i)]{scholze:relative_p-adic_hodge_theory} shows that for any $\bB_\deR^+$-local system~$\bM$ on~$U$, the natural map $\eta_\bM\colon\bM\to\rF^0(\cO\bB_{\deR,U}\otimes_{\bB_{\deR,U}^+}\bM)^{\nabla=0}$ is an isomorphism. Thus the image of the functor $\cO\bB_{\deR,U}\otimes_{\bB_{\deR,U}^+}(-)\colon\Loc_{\bB_\deR^+}(U)\to\FMIC_{\cO\bB_\deR}(U)$ has image contained in~$\dI$.

Now the construction~$\dM\mapsto\rF^0\!\dM^{\nabla=0}$ provides a functor $\dI\to\Loc_{\bB_\deR^+}(U)$ which is right adjoint to the functor $\cO\bB_{\deR,U}\otimes_{\bB_{\deR,U}^+}(-)$. The unit of this adjunction is the natural isomorphism $\eta_\bM$ above, which implies that the functor $\cO\bB_{\deR,U}\otimes_{\bB_{\deR,U}}(-)$ is fully faithful.

\smallskip

Then the proof of \cite[Theorem~7.6(ii)]{scholze:relative_p-adic_hodge_theory} shows that for every filtered vector bundle with flat connection~$\dE$, there is a $\bB_\deR^+$-local system~$\bM$ such that $\cO\bB_{\deR,U}\otimes_{\cO_U}\dE$ is isomorphic to $\cO\bB_{\deR,U}\otimes_{\bB_{\deR,U}^+}\bM$ compatibly with the filtrations and connection. This says that the essential image of the functor $\cO\bB_{\deR,U}\otimes_{\cO_U}(-)\colon\FMIC(U)\to\FMIC_{\cO\bB_\deR}(U)$ is contained in the essential image of the functor $\cO\bB_{\deR,U}\otimes_{\bB_{\deR,U}^+}(-)\colon\Loc_{\bB_\deR^+}(U)\to\FMIC_{\cO\bB_\deR}(U)$. The fact that the functor $\dE\mapsto\cO\bB_{\deR,U}\otimes_{\cO_U}\dE$ is fully faithful follows then from the fact that the composite functor $\dE\mapsto\rF^0\!(\cO\bB_{\deR,U}\otimes_{\cO_U}\dE)^{\nabla=0}$ is fully faithful \cite[Theorem~7.6(ii)]{scholze:relative_p-adic_hodge_theory}.
\end{proof}
\end{prop}

\begin{rmk}
In \cite{scholze:relative_p-adic_hodge_theory}, Scholze does not work with filtered $\cO\bB_\deR$-modules with flat connection: instead, he uses $\cO\bB_\deR^+$-modules with flat connection \cite[Definition~7.1(ii)]{scholze:relative_p-adic_hodge_theory} where $\cO\bB_{\deR,U}^+$ is the positive structural de Rham period sheaf \cite[Definition~6.8(iii)]{scholze:relative_p-adic_hodge_theory}\cite[Erratum~(3)]{scholze:relative_p-adic_hodge_theory_erratum}. The advantage of Scholze's approach is that the functor $\cO\bB_{\deR,U}^+\otimes_{\bB_{\deR,U}^+}(-)$ from $\bB_\deR^+$-local systems on~$U$ to $\cO\bB_\deR^+$-modules with flat connection is then an equivalence \cite[Theorem~7.2]{scholze:relative_p-adic_hodge_theory} -- this is a $p$-adic version of the Riemann--Hilbert correspondence. On the other hand, defining a functor directly from $\FMIC(U)$ to $\MIC_{\cO\bB_\deR^+}(U)$ is not as simple as just base-changing along a morphism of sheaves of rings, so in the interest of simplicity of exposition, we have chosen to focus on the category of filtered $\cO\bB_\deR$-modules with flat connection instead.
\end{rmk}

The $\otimes$-functors~\eqref{eq:base-change_functors} allow one to isolate an important class of $\hat\bZ_p$-local systems on~$U$, namely those for which there is a corresponding filtered vector bundle with flat connection under~\eqref{eq:base-change_functors}.

\begin{defi}
	A \emph{de Rham pair} on~$U$ is a triple $(\bL,\dE,c_\deR)$ consisting of a $\hat\bZ_p$-local system~$\bL$ on~$U$, a filtered vector bundle with flat connection~$\dE$ on~$U$, and an isomorphism
	\[
	c_\deR\colon \cO\bB_{\deR,U}\otimes_{\hat\bZ_{p,U}}\bL\xrightarrow\sim\cO\bB_{\deR,U}\otimes_{\cO_U}\dE
	\]
	of filtered $\cO\bB_{\deR,U}$-modules with flat connection on~$U$. The collection of all de Rham pairs naturally forms a $\bZ_p$-linear abelian $\otimes$-category, the precise formulation of which we leave to the reader.
	
	It follows from Proposition~\ref{prop:p-adic_riemann-hilbert} that the forgetful functor from de Rham pairs to $\hat\bZ_p$-local systems on~$U$ is fully faithful. We say that a $\hat\bZ_p$-local system~$\bL$ is \emph{de Rham} just when it lies in the essential image of this functor, i.e.\ just when~$\bL$ is the first component of a de Rham pair $(\bL,\dE,c_\deR)$.
\end{defi}

\begin{rmk}
	A $\hat\bZ_p$-local system~$\bL$ and filtered vector bundle~$\dE$ appearing in a de Rham pair $(\bL,\dE,c_\deR)$ are said to be \emph{associated} \cite[Definition~8.3]{scholze:relative_p-adic_hodge_theory}. The reason we introduce the category of de Rham pairs is that, for our purposes, it will be necessary not just to keep track of whether~$\bL$ and~$\dE$ are associated, but also to keep track of the isomorphism~$c_\deR$ which relates them.
\end{rmk}

\subsubsection{Pullback of de Rham pairs}

The theory described above is contravariant-functorial in the smooth $K_v$-analytic space~$U$ in a natural way. Suppose that $f\colon V\to U$ is a morphism of smooth rigid-analytic spaces over~$K_v$. This induces a morphism $f\colon V_\proet\to U_\proet$ on pro-\'etale sites, and there are morphisms of sheaves of $\bZ_p$-algebras
\begin{align*}
	f^{-1}\hat\bZ_{p,U} &\to \hat\bZ_{p,V} & f^{-1}\bB_{\deR,U}^+ &\to \bB_{\deR,V}^+ \\
	f^{-1}\cO_U &\to \cO_V & f^{-1}\cO\bB_{\deR,U} &\to \cO\bB_{\deR,V}
\end{align*}
compatible with all structures. Via these maps, we obtain pullback $\otimes$-functors\footnote{We denote all of these different functors by the same symbol $f^*$. It should always be clear from context which of these functors we mean in any given instance.}
\begin{align*}
	f^*\colon\Loc_{\hat\bZ_p}(U) &\to \Loc_{\hat\bZ_p}(V) & f^*\colon\Loc_{\bB_\deR^+}(U) &\to \Loc_{\bB_\deR^+}(V) \\
	f^*\colon\FMIC(U) &\to \FMIC(V) & f^*\colon\FMIC_{\cO\bB_\deR}(U) &\to \FMIC_{\cO\bB_\deR}(V) \,.
\end{align*}

The following is easily verified.

\begin{prop}
	Let~$f\colon V\to U$ be a morphism of smooth $K_v$-analytic spaces, and suppose that $(\bL,\dE,c_\deR)$ is a de Rham pair on~$U$.
	
	Then the solid arrows in the diagram
	\begin{center}
		\begin{tikzcd}
			\cO\bB_{\deR,V}\otimes_{\hat\bZ_{p,V}}f^*\bL \arrow[r,dashed]\arrow[d,"\wr"] & \cO\bB_{\deR,V}\otimes_{\cO_V}f^*\dE \arrow[d,"\wr"] \\
			f^*(\cO\bB_{\deR,U}\otimes_{\hat\bZ_{p,U}}\bL) 
			\arrow[r,"f^*c_\deR","\sim"'] & f^*(\cO\bB_{\deR,U}\otimes_{\cO_U}\dE)
		\end{tikzcd}
	\end{center}
	are all isomorphisms of filtered $\cO\bB_\deR$-modules on~$V$. We write~$f^*(\bL,\dE,c_\deR)$ for the de Rham pair $(f^*\bL,f^*\dE,\tilde c_\deR)$ on~$V$, where~$\tilde c_\deR$ is the unique dashed arrow making the above square commute.
\end{prop}

\subsubsection{Derived pushforward of de Rham pairs}

In certain circumstances, it is also possible to push forward local systems and filtered vector bundles with flat connection along morphisms $\pi\colon V\to U$ of smooth $K_v$-analytic spaces. Suppose that~$\pi$ is smooth and proper.

Since the category of sheaves of abelian groups on~$V_\proet$ is Grothendieck abelian, it has enough K-injectives \todo{cite}, and so the pushforward functor~$\pi_*$ has a total derived functor $\rR\!\pi_*\colon\Derv\Sh(V_\proet)\to\Derv\Sh(U_\proet)$ between the unbounded derived categories of sheaves on~$U_\proet$ and~$V_\proet$. This functor is lax symmetric monoidal, meaning that it comes with natural maps
\begin{align*}
\rR\!\pi_*\dF^\bullet\Lotimes_{\uZ_U}\rR\!\pi_*\dG^\bullet &\to \rR\!\pi_*(\dF^\bullet\Lotimes_{\uZ_V}\dG^\bullet) \\
\uZ_U &\to \rR\!\pi_*\uZ_V
\end{align*}
in $\Derv\Sh(U_\proet)$ which are compatible with the associativity, commutativity and unitality constraints on~$\Derv\Sh(U_\proet)$ and~$\Derv\Sh(V_\proet)$.

This implies in particular that the derived pushforward $\rR^i\!\pi_*\bL$ of a $\hat\bZ_{p,V}$-module~$\bL$ canonically has the structure of a $\hat\bZ_{p,U}$-module, induced from restricting the action map
\[
\rR\!\pi_*\hat\bZ_{p,V}\Lotimes_{\uZ_U}\rR\!\pi_*\bL\to\rR\!\pi_*(\bZ_{p,V}\Lotimes_{\uZ_V}\bL)\to\rR\!\pi_*\bL
\]
along the morphisms
\[
\hat\bZ_{p,U}\to\pi_*\hat\bZ_{p,V}\to\rR\!\pi_*\hat\bZ_{p,V}
\]
of rings in $\Derv\Sh(U_\proet)$. Note that even if~$\bL$ is a $\hat\bZ_p$-local system on~$V$, the derived pushforward~$\rR^i\!\pi_*\bL$ need not necessarily be a $\hat\bZ_p$-local system on~$U$.
\alex{24/3}{I'm not 100\% sure this is okay here: are we not using some kind of flatness?}
\smallskip

If instead~$\dE$ is a filtered vector bundle with flat connection on~$V$, then it has an associated \emph{relative de Rham complex}
\[
\DeR_{V/U}(\dE):=\dE\xrightarrow\nabla\Omega^1_{V/U}\otimes_{\cO_V}\dE\xrightarrow\nabla\Omega^2_{V/U}\otimes_{\cO_V}\dE\xrightarrow\nabla\dots
\]
defined e.g.\ as in \todo{cite}. The \emph{derived de Rham pushforward} $\rR^i\!\pi_{\deR*}\dE:=\rR^i\!\pi_*\DeR_{V/U}(\dE)$ of~$\dE$ is defined to be the $i$th cohomology object of the derived pushforward of the relative de Rham complex. Since the relative de Rham complex is a complex of~$\pi^{-1}\cO_U$-modules, it follows as above that $\rR^i\!\pi_{\deR*}\dE$ canonically has the structure of a $\cO_U$-module.

The relative de Rham complex carries a natural filtration defined by
\[
\rF^i\DeR_{V/U}(\dE) := \rF^i\!\dE \xrightarrow\nabla \Omega^1_{V/U}\otimes_{\cO_U}\rF^{i-1}\!\dE \xrightarrow\nabla \Omega^2_{V/U}\otimes_{\cO_U}\rF^{i-2}\!\dE \xrightarrow\nabla \dots \,,
\]
which endows $\rR\!\pi_{\deR*}\dE$ with the structure of an object in the filtered derived category of sheaves on~$U_\proet$ (see e.g.\ \cite[Chapter~I.3]{huber:mixed_motives} for definitions). In particular, each $\rR^i\!\pi_{\deR*}\dE$ carries a filtration by $\cO_U$-submodules. \todo{?}

\alex{19.02.2021}{I'm not entirely happy with the explanation above. Is it clear that these definitions agree with the ones that Scholze uses in his paper? I would also like to understand this filtration better, and whether these cohomology groups can be computed via \u Cech cohomology.}

\todo{explain carefully how to push forward everything}

\begin{thm}[{\cite[Theorem~1.10]{scholze:relative_p-adic_hodge_theory}}]\label{thm:pushforward_of_pairs}
	Let $\pi\colon V\to U$ be a smooth proper morphism of smooth rigid-analytic spaces over~$K_v$, and let~$(\bL,\dE,c_\deR)$ be a de Rham pair on~$V$. Suppose that the derived pushforward~$\rR^i\!\pi_*\bL$ is a $\hat\bZ_p$-local system on~$U$. Then $\rR^i\!\pi_{\deR*}\dE$ is a filtered vector bundle with flat connection on~$U$, and the solid maps in the diagram
	\begin{center}
		\begin{tikzcd}[column sep = large]
			\cO\bB_{\deR,U}\otimes_{\hat\bZ_{p,U}}\rR^i\!\pi_*\bL \arrow[r,dashed]\arrow[d,"\wr"] & \cO\bB_{\deR,U}\otimes_{\cO_U}\rR^i\!\pi_{\deR*}\dE \arrow[d,"\wr"] \\
			\rR^i\!\pi_{\deR*}(\cO\bB_{\deR,V}\otimes_{\hat\bZ_{p,V}}\bL) \arrow[r,"\rR^i\!\pi_{\deR*}c_\deR","\sim"'] & \rR^i\!\pi_{\deR*}(\cO\bB_{\deR,V}\otimes_{\cO_V}\dE)
		\end{tikzcd}
	\end{center}
	are all isomorphisms of filtered $\cO\bB_\deR$-modules on~$U$. We write $\rR^i\!\pi_*(\bL,\dE,c_\deR)$ for the de Rham pair $(\rR^i\!\pi_*\bL,\rR^i\!\pi_{\deR*}\dE,\tilde c_\deR)$ on~$U$, where~$\tilde c_\deR$ is the unique dashed arrow making the above square commute.
	\begin{proof}
		\todo{check proof}
		Strictly speaking, the statement of \cite[Theorem~1.10]{scholze:relative_p-adic_hodge_theory} only asserts that there exists an isomorphism $\cO\bB_{\deR,U}\otimes_{\hat\bZ_{p,U}}\rR^i\!\pi_*\bL\xrightarrow\sim\cO\bB_{\deR,U}\otimes_{\cO_U}\rR^i\!\pi_{\deR*}\dE$. However, the proof in fact establishes the more precise statement above, namely that the vertical arrows are isomorphisms.
	\end{proof}
\end{thm}

\subsubsection{Horizontal de Rham local systems}

\alex{24/3}{This needs to be written up, summarising Shimizu's theory}

\subsubsection{Proof of Theorem~\ref{thm:period_maps_control_reps}}\label{sss:proof_of_period_maps}

Now we finally come to the proof of Theorem~\ref{thm:period_maps_control_reps}. Let~$\pi\colon X\to Y$ be a smooth proper morphism of smooth $K_v$-varieties, as in the setup of Theorem~\ref{thm:period_maps_control_reps}. We write
\[\bL := \rR^i\!\pi^\an_*\hat\bZ_{p,X^\an}
\hspace{0.4cm}\text{and}\hspace{0.4cm}
\dE := \rR^i\!\pi^\an_{\deR*}\cO_{X^\an}\]
for the relative analytic pro-\'etale and de Rham cohomology, respectively. These are the analytifications of the corresponding analytic objects.

\begin{lem}\label{lem:analytic_is_algebraic_analytified}
	There are canonical isomorphisms
	\[
	\bL \cong \varprojlim\left(\rR^i\!\pi_*\underline{\bZ/p^n\bZ}_X\right)^\an
	\hspace{0.4cm}\text{and}\hspace{0.4cm}
	\dE \cong \cH^i_\deR(X/Y)^\an
	\]
	where $(-)^\an$ stands for pullback along the morphism of sites $Y^\an_\proet\to Y_\et$ (with appropriate sheaves of rings).
	\begin{proof}
		See \cite[\S9]{scholze:relative_p-adic_hodge_theory}.
	\end{proof}
\end{lem}

Since each derived pushforward $\rR^i\!\pi_*\underline{\bZ/p^n\bZ}_X$ is a $\bZ/p^n\bZ$-local system on~$Y$, it follows from Lemma~\ref{lem:analytic_is_algebraic_analytified} that~$\bL$ is a $\hat\bZ_p$-local system on~$Y^\an$, and hence Scholze's relative comparison theorem (Theorem~\ref{thm:pushforward_of_pairs}, applied to the de Rham pair $(\hat\bZ_{p,X^\an},\cO_{X^\an},\id)$) implies that~$\bL$ is de Rham, and comes with a canonical comparison isomorphism
\begin{equation}\label{eq:relative_comparison}
c_\deR\colon\cO\bB_{\deR,Y^\an}\otimes_{\hat\bZ_{p,Y^\an}}\bL \xrightarrow\sim \cO\bB_{\deR,Y^\an}\otimes_{\cO_{Y^\an}}\dE
\end{equation}
of filtered $\cO\bB_\deR$-vector bundles with flat connection on~$Y^\an$.
\smallskip

Now for any point~$y\in Y(K_v)$, the base change theorems for algebraic \'etale and de Rham cohomology provide isomorphisms
\begin{equation}\label{eq:fibres_of_relative_cohomology}
\rH^i_\et(X_{y,\Kbar_v},\bZ_p) \cong \bL_y \hspace{0.4cm}\text{and}\hspace{0.4cm} \rH^i_\deR(X_y/K_v) \cong \dE_y
\end{equation}
compatible with the Galois action and Hodge filtration, respectively, using Lemma~\ref{lem:analytic_is_algebraic_analytified}. These identifications are moreover compatible with the comparison isomorphisms.

\begin{lem}\label{lem:fibres_of_relative_comparison_iso}
	For every~$y\in Y(K)$, the isomorphisms of~\eqref{eq:fibres_of_relative_cohomology} fit into a commuting square
	\begin{center}
	\begin{tikzcd}
		\sB_\deR\otimes_{\bZ_p}\rH^i_\et(X_{y,\Kbar_v},\bZ_p) \arrow[r,"\sim"]\arrow[d,"c_\deR"',"\wr"] & \left(\cO\bB_{\deR,Y^\an}\otimes_{\hat\bZ_{p,Y^\an}}\bL\right)_y \arrow[d,"c_{\deR,y}","\wr"'] \\
		\sB_\deR\otimes_{K_v}\rH^i_\deR(X_y/K_v) \arrow[r,"\sim"] & \left(\cO\bB_{\deR,Y^\an}\otimes_{\cO_{Y^\an}}\dE\right)_y
	\end{tikzcd}
	\end{center}
	where the left-hand vertical arrow is the comparison isomorphism \todo{insert reference} and the right-hand vertical arrow is the fibre of~\eqref{eq:relative_comparison} at~$y$.
	\begin{proof}
		\alex{24/3}{This is what I want to prove by being careful about Scholze's constructions}
	\end{proof}
\end{lem}

Now suppose that~$\Nbd\subseteq Y^\an$ is an admissible open, isomorphic to a closed polydisc, over which~$\dE$ has a full basis of horizontal sections. Thus for any point~$y_0\in \Nbd(K_v)$ we have the parallel transport map
\[
T_{y_0}^\nabla\colon \cO_\Nbd\otimes_{K_v}\dE_{y_0} \xrightarrow\sim \dE
\]
uniquely characterised by the fact that it is $\cO_\Nbd$-linear, compatible with the connection, and restricts to the identity at~$y_0$. The parallel transport map induces, via the comparison isomorphism~\eqref{eq:relative_comparison}, another map
\[
T_{y_0}^\nabla\colon \cO\bB_{\deR,\Nbd}\otimes_{\bZ_p}\bL_{y_0} \xrightarrow\sim \cO\bB_{\deR,\Nbd}\otimes_{\hat\bZ_{p,\Nbd}}\bL
\]
which we continue to denote by the same symbol. Since $\Gamma(\Nbd,\cO\bB_{\deR,U})^{\nabla=0}=K_v$ by \cite[Corollary~6.19]{scholze:relative_p-adic_hodge_theory}, this latter map is uniquely characterised by the fact that it is $\cO\bB_{\deR,\Nbd}$-linear, compatible with the connection, and restricts to the identity at~$y_0$.

By mild abuse of notation, for another point~$y\in\Nbd(K_v)$, we denote by
\[
T_{y_0,y}^\nabla\colon \rH^i_\deR(X_{y_0}/K_v) \xrightarrow\sim \rH^i_\deR(X_y/K_v)
\hspace{0.4cm}\text{and}\hspace{0.4cm}
T_{y_0,y}^\nabla\colon \sB_\deR\otimes_{\bQ_p}\rH^i_\et(X_{y_0,\Kbar_v},\bQ_p) \xrightarrow\sim \sB_\deR\otimes_{\bQ_p}\rH^i_\et(X_{y,\Kbar_v},\bQ_p)
\]
the fibres of the above maps~$T_{y_0}^\nabla$ at~$y$, after we identify the fibres of $\dE$ and~$\bL$ using~\eqref{eq:fibres_of_relative_cohomology}. It follows immediately from Lemma~\ref{lem:fibres_of_relative_comparison_iso} that these parallel transport maps are compatible with the de Rham comparison isomorphism.

\begin{lem}
	For every~$y_0,y\in\Nbd$, the square
	\begin{center}
	\begin{tikzcd}
		\sB_\deR\otimes_{\bQ_p}\rH^i_\et(X_{y_0,\Kbar_v},\bQ_p) \arrow[r,"c_\deR","\sim"']\arrow[d,"T_{y_0,y}^\nabla"',"\wr"] & \sB_\deR\otimes_{K_v}\rH^i_\deR(X_{y_0}/K_v) \arrow[d,"T_{y_0,y}^\nabla","\wr"'] \\
		\sB_\deR\otimes_{\bQ_p}\rH^i_\et(X_{y,\Kbar_v},\bQ_p) \arrow[r,"c_\deR","\sim"'] & \sB_\deR\otimes_{K_v}\rH^i_\deR(X_y/K_v)
	\end{tikzcd}
	\end{center}
	commutes.
\end{lem}

Moreover, we know from Shimizu's theory that the parallel transport map
\[
T_{y_0,y}^\nabla\colon \sB_\deR\otimes_{\bQ_p}\rH^i_\et(X_{y_0,\Kbar_v},\bQ_p) \xrightarrow\sim \sB_\deR\otimes_{\bQ_p}\rH^i_\et(X_{y,\Kbar_v},\bQ_p)
\]
is a morphism of~$(\varphi,N,G_v)$-modules, in the following sense.

\begin{lem}\label{lem:parallel_transport_is_B_st-linear}
	For every~$y_0,y\in U$, the parallel transport map
	\[
	T_{y_0,y}^\nabla\colon\sB_\deR\otimes_{\bQ_p}\rH^i_\et(X_{y_0,\Kbar_v},\bQ_p) \xrightarrow\sim \sB_\deR\otimes_{\bQ_p}\rH^i_\et(X_{y,\Kbar_v},\bQ_p)
	\]
	restricts to a $\sB_\st$-linear isomorphism
	\[
	T_{y_0,y}^\nabla\colon\sB_\st\otimes_{\bQ_p}\rH^i_\et(X_{y_0,\Kbar_v},\bQ_p) \xrightarrow\sim \sB_\st\otimes_{\bQ_p}\rH^i_\et(X_{y,\Kbar_v},\bQ_p)
	\]
	commuting with the $(\varphi,N,G_v)$-action (trivial~$\varphi$ and~$N$ on~$\rH^i_\et$).
	\begin{proof}
		\alex{24/3}{I think in the end I will try to subsume this lemma into the Shimizu section, and discuss there parallel transport for de Rham local systems in a bit more detail}
	\end{proof}
\end{lem}

Taking fixed points under open subgroups of~$G_v$, we obtain from Lemma~\ref{lem:parallel_transport_is_B_st-linear} an isomorphism
\[
T_{y_0,y}^\nabla\colon \sD_\pst\left(\rH^i_\et(X_{y_0,\Kbar_v},\bQ_p)\right) \xrightarrow\sim \sD_\pst\left(\rH^i_\et(X_{y,\Kbar_v},\bQ_p)\right)
\]
of~$(\varphi,N,G_v)$-modules. We will show that this map makes the rectangle in Theorem~\ref{thm:period_maps_control_reps} commute. The map~$T_{y_0,y}^\nabla$ fits into a commuting diagram
\begin{center}
\begin{tikzcd}
	\sB_\deR\otimes\sD_\pst\left(\rH^i_\et(X_{y_0,\Kbar_v},\bQ_p)\right) \arrow[r,"\sim"]\arrow[d,"T_{y_0,y}^\nabla"',"\wr"] & \sB_\deR\otimes\rH^i_\et(X_{y_0,\Kbar_v},\bQ_p) \arrow[r,"c_\deR","\sim"']\arrow[d,"T_{y_0,y}^\nabla"',"\wr"] & \sB_\deR\otimes\rH^i_\deR(X_{y_0}/K_v) \arrow[d,"T_{y_0,y}^\nabla","\wr"'] \\
	\sB_\deR\otimes\sD_\pst\left(\rH^i_\et(X_{y_0,\Kbar_v},\bQ_p)\right) \arrow[r,"\sim"] & \sB_\deR\otimes\rH^i_\et(X_{y,\Kbar_v},\bQ_p) \arrow[r,"c_\deR","\sim"'] & \sB_\deR\otimes\rH^i_\deR(X_y/K_v)
\end{tikzcd}
\end{center}
where the unmarked horizontal arrows are the isomorphisms induced from the inclusions $\sD_\pst(-)\subseteq\sB_\st\otimes(-)\subseteq\sB_\deR\otimes(-)$. The outer rectangle in this diagram is the base change to~$\sB_\deR$ of the rectangle in Theorem~\ref{thm:period_maps_control_reps}. Thus the rectangle in Theorem~\ref{thm:period_maps_control_reps} commutes after base change along the field extension $\sB_\deR/\Kbar_v$, so is already commutative. This is what we want to show.\qed
